FedDC: Federated Learning with Non-IID Data via Local Drift Decoupling and Correction

Federated learning (FL) allows multiple clients to collectively train a high-performance global model without sharing their private data. However, the key challenge in federated learning is that the clients have significant statistical heterogeneity among their local data distributions, which would cause inconsistent optimized local models on the client-side. To address this fundamental dilemma, we propose a novel federated learning algorithm with local drift decoupling and correction (FedDC). Our FedDC only introduces lightweight modifications in the local training phase, in which each client utilizes an auxiliary local drift variable to track the gap between the local model parameter and the global model parameters. The key idea of FedDC is to utilize this learned local drift variable to bridge the gap, i.e., conducting consistency in parameter-level. The experiment results and analysis demonstrate that FedDC yields expediting convergence and better performance on various image classification tasks, robust in partial participation settings, non-iid data, and heterogeneous clients.

==> tex_file/FLN.tex <==

\section{Proposed Method}
\label{Sec_method}

\begin{comment}
This section introduces the new algorithm FedDC, and we build intuition into how it solves gradient drift and parameter drift.
\end{comment} 


\begin{comment}
We assume that there are $m$ clients to train a global model with the coordination of a central server, in which each client $i, \forall i\in [m]$ contains its local private dataset $D_i$.
\end{comment}


% \begin{wrapfigure}{R}{0.55\textwidth}
% \vspace{-15pt}
\begin{algorithm}[htbp]
\label{algorithmFedDC}
\small
	\caption{Algorithm of FedDC }
	\KwIn{Initial model $\Theta^0=\theta_i^0$, training round $T$, number of clients $m$, local drift variables $h_i^0=0,\forall i\in [m]$, local batch number  $K$.}
	\KwOut{The trained global model $\Theta^T$.}
	%\State some description 
	\For{ $t = 1,2,...,T$}{
		\textbf{Sample} the active client set $C_t\subseteq [m]$.\\ 
		\For{on each client $i \in{C_t}$ in parallel}{
			\textbf{Initialize}  $\theta_i^{t,0}=\Theta^{t-1},$\\
			\For{ $k = 1,2,...,K$}{ 
				\textbf{Update} local objective function \\ $\quad\quad$ $\arg\min_\theta F_i(\theta_i)$ in Eq.~(\ref{local_loss_1}).\\
				\textbf{Update} local model as:\\ $\quad\quad$ $\theta_i^{t,k}=\theta_i^{t,k-1}-\eta\nabla_{\theta}F_i(\theta_i^{t,k-1}). $
			}
			\textbf{Update} drift variables $h_i^t = h_i^{t-1}+\Delta\theta_i^t,$ \\ 
			$\quad\quad$ and set $\Delta\theta_i^t=\theta_i^{t}-\theta_i^{t,0}.$
		}
		\textbf{Update} server model as:\\ $\quad\quad$ $\Theta^t=\frac{1}{|C_t|}\sum\limits_{i\in C_t}(\theta_i^{t,K}+h_i^t),$\\ 
		$\quad\quad$ and set $\Delta\theta^t=\frac{1}{|C_t|}\sum\limits_{i\in C_t}\Delta\theta_i^t$.\\
	}
\end{algorithm}
% \vspace{-0.4cm}
% \end{wrapfigure}


%
In this section, we introduce the proposed FedDC algorithm. Specifically, we first present the overview of FedDC, and then discuss the local-decoupling and correction process in detail. 

\textbf{Overview.} In this work, we assume that there are $m$ active clients to train a global model with the coordination of a central server. Each client $i, \forall i\in [m]$ contains local training dataset $D_i$. Algorithm~\ref{algorithmFedDC} shows the workflow of our FedDC. In each training round, the active clients first update local models and the corresponding auxiliary drift variables in parallel, and then the server aggregates the local models and drift variables to update the global model.
FedDC does not directly adopt the average of clients' local parameters as the global parameter. Instead, FedDC decouples the global model and local models with drift variables. Each client's drift variable represents the parameter drift between its local model and the global model. We design a dynamic local objective function for each client, which contains a parameter correction term to control the parameter drift, a gradient correction term to reduce the gradient drift and an empirical loss term to minimize the expected empirical loss on the local dataset. The global objective in FedDC is to obtain a global model that minimizes the global empirical loss:
\begin{equation}\label{global_loss}
\Theta^*=\arg\min_{\Theta} \left\{F(\Theta)= \mathbb{E}_{(x,y)\in D} l(\Theta,(x,y))\right\},
\end{equation}
where $F$ is the global objective function, $(x,y)$ is the training sample $x$ and its corresponding ground-truth label $y$, $l$ represents the empirical loss function which measures the inconsistency between the predicted value of the model and the corresponding ground-truth label. The global data set $D$ is the mixture of all local data $D_i$, which can be represented as $D=\cup\{D_i\}, \forall i\in [m]$. %For each client $i\in[m]$, we assume the sample in its local data set $(x,y)\in D_i\sim P_i$ distribution, and the sample in global dataset $(x,y)\in D \sim P$ distribution.


\textbf{Decoupling local parameters and global parameters.} %In federated learning, the computing must be offload to clients in the optimization process. 
The previous FL methods~\cite{mcmahan2017communication,li2020federated,karimireddy2021scaffold} regard the local parameters in participated clients as the approximation of the global model parameters, as $\theta_i\approx\Theta,\forall i\in [m]$, where $\theta_i$ represents the parameters of the local model on the $i$-th client. However, using a single model to minimizes the local empirical losses and the global empirical loss is impractical, because the
data heterogeneity causes inconsistency on their objectives. Forcibly aligning the objectives can only result in a sub-optimal solution.
In FedDC, we decouple local parameters and the global parameter with drift variables. For client $i$, it exists a drift variable $h_i$ which represents the parameter deviation ($h_i=\Theta-\theta_i$) between the global parameters $\Theta$ and local parameters $\theta_i$.  
The local parameter $\theta_i$ focuses on optimizing the local empirical loss of client $i$, while the global parameter $\Theta$ optimizes the global empirical loss.
Thus, under ideal circumstances, the global model's parameters $\Theta$ can be represented as a decoupled sum of the local models' parameter and the corresponding drift variable for each client, $\Theta=h_i+\theta_i, \forall i$. We redefine the global objective function of Eq.~(\ref{global_loss}) with $(\theta_i,h_i)$ as:
\begin{equation}\label{seperate_loss}
F(\Theta)=F(\theta_i,h_i), \quad where \quad \Theta=\theta_i+h_i,  \forall i\in{[m]},
\end{equation}
the definition in above equation is independent of $i$, where $\theta_i$ can be optimized with clinet $i$'s local objective function according to its definition to bypass the request of aggregating all data.


%$\theta_i$ is $i$-th client's local parameters, which minimizes the empirical local objective function.

%It is worth noting that FedDC uses ($\theta_i$ + $h_i$) $\forall i\in [m]$ to approximate replace the $\Theta$ in $L_c$, while the previous methods like FedAvg in which the global objective function is the average of clients' local objective functions where $L(\Theta,D)=\sum_{i=0}^m L(\Theta,D_i)$.


%In FedDC, clients' local objective functions aims to minimize the local empirical losses and fit the current state in each round. The 
\textbf{Dynamic local objective function.}
In FedDC, each client's local objective function contains a local empirical loss, a gradient correction term and a parameter correction term. For client $i$, the local objective function in $t$-th round is:
% \begin{equation}\label{local_loss_1}
% F_i(\theta_i)= \mathbb{E}_{(x,y)\in D_i}l(\theta_i,(x,y)) +\frac{\alpha}{2} ||\theta_i-(\Theta^{t-1}-{h}_i^{t-1})||^2  + \frac{1}{K\eta} \langle\theta_i,\Delta\theta_i^{t-1}-\Delta\theta^{t-1}\rangle,
% \end{equation}


\begin{gather}
F_i(\theta_i)= \mathbb{E}_{(x,y)\in D_i}l(\theta_i,(x,y)) +\frac{\alpha}{2} ||\theta_i-(\Theta^{t-1}-{h}_i^{t-1})||^2   \notag\\
+ \frac{1}{K\eta} \langle\theta_i,\Delta\theta_i^{t-1}-\Delta\theta^{t-1}\rangle,
\end{gather}


where the first term $\mathbb{E}_{(x,y)\in D_i}l(\theta_i,(x,y))$ is the empirical loss on local client. The second term $\frac{\alpha}{2} ||\theta_i-(\Theta^{t-1}-{h}_i^{t-1})||^2$ is a parameter correction term which regulate the local parameter $\theta_i$ close to drift corrected parameter $\Theta-h_i$, $\alpha$ is a hyper-parameter. In addition, in order to reduce the gradient drift, we add the gradient correction term following the inspiration of Scaffold~\cite{karimireddy2021scaffold}, that is $\frac{1}{K\eta} \langle\theta_i,\Delta\theta_i^{t-1}-\Delta\theta^{t-1}\rangle$, where $\Delta\theta_i^{t-1}=\sum_{k=1}^K \Delta \theta_i^{t-1,k}=-\eta\sum_{k=1}^K\nabla_\theta F_i(\theta_i^{t-1,k})$ and $\Delta\theta^{t-1}=\mathbb{E}\Delta\theta_i^{t-1}$, $\eta$ is the learning rate and $K$ is the number of local training iterations in one training round. 
% \textcolor{red}{better to write some rationale about the design.}

%We expand the second term in Equation \ref{local_loss_1} and keep only the items related to the parameter $\theta_i$ to be optimized. In addition, in order to reduce the update difference between customers, we have added gradient correction items following the Scaffold method, that is $\frac{1}{K\eta} \langle\theta_i,\Delta\theta_i^{t-1}-\Delta\theta^{t-1}\rangle$. $K$ is the number of local training iterations in one communication round.
%The local objective function of client $i,\forall i\in [m]$ in FedDC is the sum of an empirical loss, a proximal regularization term, a regularization term and a gradient correction term:
%\begin{equation}\label{local_loss}
%L_i(\theta_i)= \mathbb{E}_{(x,y)\in D_i}l(\theta_i,(x,y)) -\alpha \langle\theta_i,\hat{\theta}_i^{t-1}\rangle  +\frac{1}{K\eta} \langle\theta_i,\Delta\theta_i^{t-1}-\Delta\theta^{t-1}\rangle+(\frac{\alpha}{2}+\beta)||\theta_i||^2,
%\end{equation}
%The local empirical loss $\mathbb{E}_{(x,y)\in D_i}l(\theta_i,(x,y)) $ aims to fit local data, the proximal regularization term $-\alpha \langle\theta_i,\hat{\theta}_i^{t-1}\rangle$ constracts the relation of local parameter with the global parameter, the gradient correction term $\langle\theta_i,\Delta\theta_i^{t-1}-\Delta\theta^{t-1}\rangle$ reduces the drift of clients' updates.

\textbf{Optimization process.}
From the definition of Eq.~(\ref{seperate_loss}), we get $\nabla_\Theta F(\Theta^t)=\nabla_\theta F(\theta_i^t,h_i^t)=\nabla_h F(\theta_i^t,h_i^t)$. So FedDC can update $\theta_i$ and $h_i$ with the same value, where $\Delta \theta_i^{t,k}=\Delta h_i^{t,k}$ always holds for $\forall t,k$.
%
Similar to most FL algorithms, FedDC also conducts multiple SGD iterations ($K>1$) in each training round in order to reduce the communication overhead. We assume the active client set in the $t$-th round is $C_t$, where $C_t \subseteq [m]$.

In the $k$-th local training iteration of the $t$-th communication round, the client first optimizes local model with the gradient of local objective function which is represented as follows:
\begin{equation}\label{local_update}
\theta_i^{t,k}=\theta_i^{t,k-1}-\eta\nabla_{\theta}F_i(\theta_i^{t,k-1}).
\end{equation}
After that, the drift variable is updated with $h_i^{t,k}=h_i^{t,k-1}+\Delta \theta_i^{t,k}=h_i^{t,k-1}-\eta\nabla_{\theta}F_i(\theta_i^{t,k})$ according to $\nabla_\theta F(\theta_i^{t,k},h_i^{t,k})=\nabla_h F(\theta_i^{t,k},h_i^{t,k})$.
The update value of local parameters in the $t$-th round can be represented as $\Delta \theta_i^t =-\eta\sum_{k=1}^K \nabla_\theta F_i(\theta_i^{t,k},h_i^{t,k})$. At the same time, the update value of the corresponding drift variable is represented as $\Delta h_i^t =h_i^{t,K}-h_i^{t,0}=-\eta\sum_{k=1}^K \nabla_\theta F_i(\theta_i^{t,k},h_i^{t,k})$.
After the local training process completes, the server updates the global parameters based on the updated $\theta_i^{t}$ and $h_i^{t}$ with the following approach:
\begin{equation}\label{update_global}
\Theta^t=\mathbb{E}_{i\in [C_t]}(\theta_i^{t}+h_i^{t})=\mathbb{E}_{i\in [C_t]}(\theta_i^{t-1}+h_i^{t-1}+\Delta \theta_i^t+\Delta h_i^t ),
\end{equation}
%where $C_t$ is the active client set in round $t$, $C_t\in [m]$, 
where $\theta_i^t$ and $h_i^t$ are short for $\theta_i^{t,K}$ and $h_i^{t,K}$, respectively. In Eq.~(\ref{update_global}), we update the global parameter with the expected value of the sum $\theta_i^t+h_i^t$ for all $i\in C_t$ instead of using $\theta_i^t+h_i^t$ of a single client $i$ to reduce the random error from local optimization. Repeating the above steps in each training round, the client $i$ will get its personalized model $\theta_i^T$ after $T$-th communication rounds.  $\theta_i^T\neq\theta_j^T$ for any $D_i\neq D_j$ for the reason that their local data distribution are different. Although the local parameters are different from each other, their global parameters reach a consistent global stationary point where $\Theta^T=\theta_i^T+h_i^T$, for $\forall i \in [m]$. 

In practice, we relax the optimization constraints on the drift variable $h_i$. Since $\nabla{h_i^{t,k}}=\nabla\theta_i^{t,k}$, $h_i$ and $\theta_i$ need not to be updated step by step. We fix $h_i$ to update $\theta_i$ for $K$ iterations in one training round, and then $h_i$ is updated with only one step in this round: $h_i^t=h_i^{t-1}+\Delta{h_i^{t}}=h_i^{t-1}+\Delta{\theta_i^t}$ to save computing resource.
In this way, the optimization process of FedDC would not consume more computing resources than a standard FedAvg. Besides, we compare the communication cost of FedDC with FedAvg in each round. A client in FedAvg uploads its local model and downloads the global model in one round. In FedDC, at the beginning of $t$-th round, client $i$ downloads $\Theta^{t-1}$ and $\Delta\theta^{t-1}$, and after local training it uploads the sum of $\theta_i^t+h_i^t$ to the server. In FedDC, other variables are calculated with the locally stored variables and the transmitted parameters above mentioned. Thus, FedDC transmits $1.5\times$ amount of data each round compared with FedAvg.
%At the end of each communication round, the server update global model's parameter as $\Theta=\mathbb{E}(\theta_i+h_i)=\frac{1}{m}\sum\limits_{i=1}^m(\theta_i+h_i)$, which is used as the new starting point at next round. For the case where only part clients participating training, we can use $\Theta=\mathbb{E}(\theta_i+h_i)=\frac{1}{m}\sum\limits_{i\in[S_t]}(\theta_i+h_i)$ to update the global model, where $S_t$ is the active client set in round $t$.


\textbf{Discussion.} The parameters of clients' local model indirectly align with global parameters by adding the drift variables. In federated learning, suppose the clients' local optimal points $\theta_i^*,\forall i\in[m]$ are arbitrarily different from each other due to the heterogeneous training data located on various clients. We show that in FedDC, when each client reaches the local optimal points, and the global model also converges to a stationary point at the same time. %Equation \ref{seperate_loss}, we assume in $t$-th round $\Theta^t-(\theta_i^t+h_i^t)=\sigma_i^t$, the implies $(\Theta^t-h_i^t)\theta_i^t-\theta_i^t=\sigma_i^t$. In local training phase, the proximal regularization term leads to $\sigma_i^{t+1}<\sigma_i^t$. With $\sigma_i^t\rightarrow \sigma_i^\infty$, it follows $\sigma_i^t\rightarrow 0$, that indicates all $\theta_i^t+h_i^t, \forall i\in[m]$ would converge to a point independent of $i$. 
Based on the Eq.~(\ref{update_global}), if the local model converges to local optima, then $\Delta \theta_i^t\rightarrow 0, \forall i\in[m]$, that implies  $\Theta^{t}=\Theta^{t-1}+\Delta\Theta^{t+1}=\Theta^{t-1}+2\Delta \theta^t=\Theta^{t-1}$. That indicates the global model also converges when clients' local models all converge to their local stationary points. 

\textbf{Parameter correction.}
The parameter correction term is mainly used to track the parameter drift. Due to the data heterogeneity among clients, it is impractical to assume that all local models converge to a consistent stationary point. In FedDC, the parameter drift specifically tracks the deviation between local models and global model.
The parameter deviation from local models to the global model is caused by the following two factors: 1) the update drift in current round, and 2) the residual parameter deviation. 
FedProx~\cite{li2020federated} and Scaffold~\cite{karimireddy2021scaffold} have proved that reducing the update drift is effective for speed up the convergence time. However, the residual parameter drift has a cumulative effect between communication rounds, making it more critical to convergence and performance of the training process.
We use auxiliary drift variables to denote the parameter deviation of the client's local model in federated learning from the unbiased global model. In this way, we decouple the training of the global model from the clients' local models. Each client updates its drift variables under the limitation of the parameter correction term $\frac{\alpha}{2}||\theta_i-(\Theta-h_i)||^2$ which ensure the effectiveness of the drift variables. 
%global parameter is the expected value of the average sum of auxiliary parameter drift variables and the local parameters.


\textbf{Gradient correction.}
To briefly and clearly illustrate the effectiveness of the gradient correction term, we first disregard the drift variable and the parameter correction term. We assume that all clients are active. Under this condition, we suppose $L_i(\theta_i^t)=\mathbb{E}_{(x,y)\in D_i}l(\theta_i,(x,y))$ and $L(\theta)=\mathbb{E}_{(x,y)\in D}l(\theta,(x,y))$. Client $i$'s corrected gradient which uses the gradient correction term satisfies $g_i^{t,k}=\nabla_\theta L_i(\theta_i^{t,k})+\frac{1}{K\eta}(\Delta \theta_i^{t-1}-\Delta\theta^{t-1})\approx \nabla_\theta L_i(\theta_i^{t,k}) +(\nabla_\theta L(\theta_i^{t-1,k})-\nabla_\theta L_i(\theta_i^{t-1,k}))$ to optimize its model instead of $\nabla_\theta L_i(\theta_i^{t,k})$.
The gradient variance is $\frac{1}{m}\sum_{i=1}^m ||g_i^{t,k}- g^{t,k}||^2$, where $g^{t,k}=\frac{1}{m}\sum_{i=1}^mg_i^{t,k} \approx \nabla F(\theta_i^t)$. Thus, the different degrees of local gradient can be expressed as 
\begin{equation}
\small
\begin{split}
\frac{1}{m}\sum_{i=1}^m ||g_i^{t,k}- g^{t,k}||^2 & \approx \frac{1}{m} \sum_{i=1}^m ||\nabla_\theta L_i(\theta_i^{t,k}) +(\nabla_\theta L(\theta_i^{t-1,k})-\nabla_\theta L_i(\theta_i^{t-1,k}))-\nabla_\theta L(\theta_i^{t,k})||^2 \\
&\leq \frac{2}{m} \sum_{i=1}^m [||\nabla_\theta L_i(\theta_i^{t,k}) -\nabla_\theta L_i(\theta_i^{t-1,k})||^2+||\nabla_\theta L(\theta_i^{t-1,k})-\nabla_\theta L(\theta_i^{t,k})||^2].
\label{lammaf15}
\end{split}
\end{equation}
The variance of the local gradients is bounded by the above inequality, which is independent of the dissimilarity of their local objective functions. With the smoothness assumption of $L$ and $L_i, (\forall i\in [m])$, their gradients would not change a lot. We deduce that the gradient of each client is strictly bounded. Thus, the gradient correction term is effective to reduce the gradient drift. 



\textbf{Convergence analysis.}
We show the convergence theoretical analysis for FedDC in convex and non-convex functions. With the drift variable to correct the global parameter, we denote $L(\cdot)$ as the global empirical loss objective and $L(\Theta)=F(\Theta)$.
We suppose the objective function is $\beta$-Lipschitz continuous gradient and $B$-local dissimilarity bounded under the $\gamma$-inexact solution assumption \cite{MLSYS2020_38af8613}, that implies the following expected objective decent in each round:
\begin{equation}{\label{lammacon1}}
\begin{split}
&\mathbb{E}_{C_t} L(\Theta^{t}) \leq L(\Theta^{t-1})-(\frac{2-2\gamma B}{\alpha}-\frac{2\beta B(1+\gamma)}{\alpha\bar\alpha}-2\beta\frac{B^2(1+\gamma)^2}{\hat\alpha^2})||\nabla L(\Theta^{t-1})||^2,
\end{split}
\end{equation}
where $\bar\alpha=\alpha-\beta_d>0$ is a constant, $C_t$ is the selected active client set in round $t$. We can use the objective function decrease to note the convergence on convex and non-convex $L(\cdot)$.
In non-convex case, assuming $\Gamma=L(\Theta^0)-L(\Theta^*)$, $p=(\frac{1}{\alpha}-(\frac{\gamma }{\alpha}-\frac{(1+\gamma)\sqrt{2}}{\bar\alpha \sqrt{C}}-
\frac{\beta (1+\gamma)}{\alpha\bar\alpha})\sqrt{1+\frac{\sigma^2}{\epsilon}}
-(\frac{\beta(1+\gamma)^2}{2\bar\alpha^2}-\frac{\beta (1+\gamma)^2(2*\sqrt{2}+2)}{\bar\alpha^2 C}))(1+\frac{\sigma^2}{\epsilon})>0$, the relation in Eq.~(\ref{lammacon1}) holds for FedDC, we get 
$\mathbb{E}_{C_t} L(\Theta^t)\leq L(\Theta^{t-1})-2p||\nabla L(\Theta^{t-1})||^2$. Giving a $\epsilon>0$, we prove that $\sum_{t=1}^T||\nabla L(\Theta^t)||^2\leq \epsilon$ when the number of communication round satisfies $T=O(\frac{\Gamma}{p\epsilon})$. If the objective functions are convex, setting $\beta_d=0,\bar\alpha=\alpha$, if $\gamma=0$, $B\leq \sqrt{C}$ and $1<<B \leq 0.5\sqrt{C}$, we have 
\begin{equation}{\label{lammacon2}} 
\mathbb{E}_{C_t} L(\Theta^t)\leq L(\Theta^{t-1})-\frac{2}{\alpha^2}[
\alpha(1-\frac{\sqrt{2}B}{\sqrt{C}})-(B+(\frac{(2\sqrt{2}+2)}{C}+\frac{1}{2})\beta B^2)]||\nabla L(\Theta^{t-1})||^2. 
\end{equation}
Let $\alpha = 6\beta B^2$, to achieve the convergence state where $\sum_{t=1}^T||\nabla L(\Theta^t)||^2\leq \epsilon$, FedDC costs $T=O(\frac{\beta B^2\Gamma}{\epsilon})$ communication rounds. 
The detailed proof is given in Appendix~\ref{appendix_proof}.





==> tex_file/FLN_new_alg.tex <==
%\begin{figure}
%	\centering
%	\includegraphics[width=1\linewidth]{./nips-figs/framework}
%	\caption{The framework of Federated learning.}
%	\label{fig_overview}
%\end{figure}

%\begin{figure}[t]
%	\centering
%	\includegraphics[width=0.8\linewidth]{./nips-figs/example}
%	%\includegraphics[width=0.8\linewidth]{egfigure.eps}
%	
%	\caption{Example of t-SNE (from MOON, I will replace it with ours.).}
%	\label{fig_tsne}
%\end{figure}

\section{Local-drift Decoupling}
\subsection{Problem Definition of Federated Learning}
In Federated Learning, we assume that there are $N$ clients from different parties. We suppose $D_i$ is client $i$'s private local dataset. The goal is to get a global model $w_*$ training over the global dataset $D=\bigcup_{i\in{[N]}} D_i$ that solves the objective: 
\begin{equation}\label{fedavg_loss}
w^*=\arg\min_{w}L(w)= \sum_{i=1}^N \frac{|D_i|}{|D|}L_i(w),
\end{equation}
where $w$ is the parameter of the global model, $L(w,D)$ is the empirical loss on the global dataset $D$, $|D_i|$ is the sample number on client $i$'s lcoal dataset $D_i$, and $L_i(w)=\mathbb{E}_{(x,y)\in D_i}l(w;(x,y))$ is the empirical loss on client $i$'s local dataset.

In order to avoid privacy leaking, any client can not share its raw data with others. So that we can not train the global model on the global dataset because it is inaccessible. McMahan et al. \cite{mcmahan2017communication} propose the classic FedAvg algorithm to coordinate multiple clients cooperatively train the global model with a central server.
%Specifically, FedAvg use the sum of the local objectives as the alternative objective of \ref{}. 
Specifically, in this typical Federated Learning method, in each training round, each client optimize its local model on the lcoal datasets, then the server takes the expectations of the local model parameters to update the global model:
\begin{equation}\label{fedavg_global}
	w= \sum_{i=1}^N \frac{|D_i|}{|D|}\theta_i,
\end{equation}
where $w$ is the global model parameters, $\theta_i$ is client $i$'s local model parameters. 
The updated global model parameters are broadcast to clients and utilized as the start point of local models in the next round.




% causes inconsistency on their objectives. 
%Forcibly aligning the objectives can only result in a sub-optimal solution.



\subsection{Motivation}
We design FedDC based on an intuitive idea: 1) there is a drift between each client's local model trained on local dataset and the global model trained on global dataset. 2) if the drift is ignored the server would get an skewed global model.


Federated learning faces the challenge of data heterogeneity.  The clients are from different parties and they collect their local data in different scenarios. Thus, the local datasets have different features and different class distributions. Federated learning relies on stochastic gradient descent (SGD), and IID sampling of training data is very important to ensure an unbiased estimate of the model. The local model trained on heterogeneous data will inevitably deviate from the ideal global model.
In the neural network trained with highly skewed non-IID data, the accuracy of FedAvg is significantly reduced \cite{NEURIPS2020_564127c0, li2020federated}, which indicates that the model aggregation method that ignores local drift leads to the deviation of the global model.

We use a simple example to show that the model parameter divergence in FedAvg is caused by the client's local drift. cannot be eliminated in the nonlinear transformation. 
In Figure \ref{fig_tsne}, we present a simple example contains two clients. We suppose that there is a non-linear transformation function $f$ (such as Sigmoid function in the activation layer) in the model. Suppose $\theta_1$ and $\theta_2$ are local parameters of client $1$ and client $2$, $w_c$ is the ideal model parameter and $w_f$ is the FedAvg model parameter. The local drifts of client $1$ and client $2$ are $(\theta_1-w_c)$ and $(\theta_2-w_c)$, separately. $x$ is a data point, the coresponding outputs on client $1$ is $y_1= f(\theta_1x)$ and $y_2= f(\theta_2x)$ on client $2$. Then we can get that the FedAvg model parameter $w_f= \frac{\theta_1+\theta_2}{2}$. The centrilized model is an ideal model which would get the ideal output, that is, $f(w_cx)=\frac{y_1+y_2}{2}$. Thus the parameter of centrilized model is $w_c=f^{-1}(\frac{y_1+y_2}{2})/x$, where $f_{-1}$ is the inverse function of $f$. Since $f$ is a non-linear function, we have $w_f\neq w_c$ and $f(w_f,x) \neq \frac{y_1+y_2}{2}$.
That indicates the global model in FedAvg is skewed, which is likely to converge slowly and with poor accuracy.

As shown above, FedAvg cannot get a global model that same as the model trained using the global dataset. FedAvg regards the local model parameters as the clients' prediction on the global model parameters, however, that leads to an inaccurate model because there is no correspondence between the model parameters of FedAvg and the expected target value in the nonlinear transformation. In heterogeneous federated learning settings, we can improve accuracy by reducing the client's prediction bias on global model parameters. In other words, we can learn the local drift between the global model and the local model, and correct it before uploading the local model to the server. This is in line with the intuition of typical federated learning.

%2) due to the local drift, the expectation of the local model parameters cannot be used as an unbiased estimate of the global model.


%Firstly, we discuss the client drift. In federated learning, clients are from different parties and they collect their local data in different scenarios. The local datasets have different features and different class distributions. The local models are separately trained on these datasets, which cause the parameter drift between them.

%We conduct a simple example to show intuition by training Lenet on the MNIST dataset. Specifically, we get four trained models and they are the centralized model, the FedAvg model, and two local models that are independently trained on the client-side.
%Figure \ref{fig_tsne} shows the t-SNE visualization. In the centralized training model, the points of the same category are more clustered and the feature boundaries of the category are more distinct.  The client models has a greater degree of feature confusion due to potential data distribution offset. This indicates that the local model has learned a worse feature representation, and its parameters have drifted from the global model. Besides, we find that the FedAvg model better separates these class because it combines the knowledge of different clients, but it is still weaker than the centralized model. %This shows that the FedAvg method constructs a biased global model.  
%These figures show that the global model and the local models produce different feature, that is, there is drift between the local model parameters and the global model parameters.

%The discrepancy further verifies that there is a gap between the local model and the global model.

%The clients even learn a worse parameter in the local training phase due to that the local model tends to over-fit the skewed and incomplete local data distribution. 


%The previous Federated Learning methods \cite{} regard the local parameters in participated clients as the approximation of the global model parameters, where using the expectation of local parameter as the global model parameter directly. 
%We indicate that using a single model to minimize the local empirical losses and the global empirical loss is impractical because of the data heterogeneity.
%However, in nonlinear transformation, the expected value of the parameter cannot be used as an unbiased estimate of the parameter.


%If the local drift and the complex transformations in the model is ignored, directly using the parameter expectations of local models to estimate the parameter of the global model as in FedAvg will lead to slow convergence and performance degradation. 

\begin{figure}[t]
	\centering
	\includegraphics[width=0.8\linewidth]{./nips-figs/222}
	%\includegraphics[width=0.8\linewidth]{egfigure.eps}
	
	\caption{Illustration of the local drift in Federated Learning with a Sigmod activation function.}
	\label{fig_tsne}
\end{figure}


%Secondly, we illustrate that the global model in FedAvg is defective because the parameter average method cannot offset the local drifts. %Zhao et al. \cite{zhao2018federated} prove
%In Figure \ref{fig_tsne}, we present a simple example contains two clients. We suppose that there is a non-linear transformation function $f$ (such as Sigmoid function in the activation layer) in the model. Suppose $w_1$ and $w_2$ are local parameters of client $1$ and client $2$, $x$ is a data point, the coresponding outputs on client $1$ is $y_1= f(w_1x)$ and $y_2= f(w_2x)$ on client $2$. Then we can get that the FedAvg model parameter $w_f= \frac{1}{2}(w_1+w_2)$, the centrilized model parameter $w_c=f^{-1}(\frac{1}{2}(y_1+y_2))/x$, where $f_{-1}$ is the inverse function of $f$. Since $f$ is a non-linear function, we have $w_f\neq w_c$ and $f(w_f,x) \neq \frac{y_1+y_2}{2}$.
%That indicates the global model in FedAvg is not the optimal model, which is likely to converge slowly and with poor accuracy.
%Therefore, under the federated learning settings, it is essential to bridge the drift between the parameters of the local model and the global model. In this paper, we introduce an auxiliary variable called the drift variable to learn and bridge the drift.

%In order to control the drift and bridge the gap between the parameters of the local model and the global model.

\section{Method}
Based on the above intuition, We propose FedDC. FedDC aims to improve the robustness and speed of model convergence by learning the model drift on the client-side and bridging the drift.
Since the features and data distributions of clients are different from the global dataset, there is always a drift between the local model parameters and the global model parameters. Local models tend to overfit on local data sets. 
In FedDC, we decouple the client's local parameters and the global parameters in the training process to avoid model over-fitting caused by ignoring model drifts. Each client uses an auxiliary variable called the local drift variable to represent the gap between its own local model and the global model. The local drift is learned in the local training phase, and in the model aggragating phase it is used to bridge the model gap.
In the following section, we introduce the objective losses and training process of FedDC in detail. 

\subsection{Objectives in FedDC}
%\subsubsection{Restriction of FedDC}
In FedDC, we denote the local drift of client $i$ as $h_i$, in an ideal condition its should satisfies the following restriction: $h_i=w-\theta_i$.
$\theta_i$ is the parameter of client $i$'local model, and $w$ is the parameter of the global model.
%that aims to minimize the empirical loss on client $i$'s local data set
% that aims to minimize the experience loss on the global data set $D$
In the whole training process, we need to keep this restriction to prevent the drift from getting out of our control. Therefore, we further convert this restriction as a penalized term, for client $i$, it is:
\begin{equation}\label{penalty_term}
R_i(\theta_i,h_i,w) =||h_i+\theta_i-w||^2, \forall i \in [N]
\end{equation}
Each client combines this penalized term with its experience loss term on the corresponding dataset to train the model parameters and the local drift variables. In this way, we transform an equation-constrained optimization problem into an unconstrained optimization problem. %The specific objectives loss is introduced in the following.


The local model parameter is the client's observation value of the global model parameter on the local dataset. The objective loss of the local model parameter is the sum of three parts: the local empirical loss term, the penalized term, and a gradient correction term. The objective loss is dynamically updated in each round based on the current global model, and the current local drift. For client $i$ ($\forall i \in [N]$), the local parameter $\theta_i$'s objective loss is:
\begin{equation}\label{local_loss}
F(\theta_i; w,h_i,D_i)=L_i(\theta_i)+ \frac{\alpha}{2}R_i(\theta_i;w_i,w) + G_i(\theta_i),
\end{equation}
where $L_i$ is $L_i$ for the typical empirical loss on $D_i$ for supervised learning, $R_i$ is the penalized term used to maintain equality of $w=\theta_i+ h_i$, $G_i$ is the gradient correction term that controll the gradient stochastic optimization. $F(\theta_i; w,h_i,D_i)$ represents in the optimization process, we optimizate $\theta_i$ on local dataset $D_i$ with $w$ and $h_i$, $L_i(\theta_i)$ fixed. 
It is worth note that the gradient correction term is proposed in Scaffold method by Karimireddy et al. \cite{karimireddy2021scaffold}.
Following Scaffold \cite{karimireddy2021scaffold}, $G_i(\theta_i)=\frac{1}{\eta K}\langle\theta_i,g_i-g\rangle,$ where $\eta$ is the learning rate, $K$ is the amount of training iterations in one round, $g_i$ is the update value of $\theta_i$ in last round, $g$ is the update value of $w$ in last round. Its role is to reduce the variance of the client gradients, we will discuss it in detail in Section \ref{sec_discussion}.

% Following Scaffold, $G_i(\theta_i)=\frac{1}{\eta K}\langle\theta_i,g_i-g\rangle,$ where $\eta$ is the learning rate, $K$ is the amount of training iterations in one round, $g_i$ is the update value of $\theta_i$ in last round, $g$ is the update value of $w$ in last round. Scaffold~\cite{karimireddy2021scaffold} have proved that reducing the update drift is effective for speed up the convergence time. 
%
%As Eq. \ref{fedavg_loss} shows, the goal of the global model parameter is to minimize the empirical loss on the global dataset $D$. Due to privacy issues, we can only train parameters on the client's local dataset. Considering the case where $w$ is trained on a single client, as the $D_i\subset D$, the global model $w$ can also fit the local data distribution of any client. 

%Thus, on client $i$, we denote the objective function of the global parameter as:$F(w| \theta_i,h_i,D_i)$. 
% $\mathbb{E}_{(x,y)\in D_i} l(w,(x,y))$. 
%\begin{equation}\label{global_loss}
%w^*=\arg\min_{w} \left\{F(w) = \mathbb{E}_{(x,y)\in D} l(w,(x,y))\right\},
%\end{equation}

%where the first term $\mathbb{E}_{(x,y)\in D_i}l(\theta_i,(x,y))$ is the empirical loss on local client. The second term $\frac{\alpha}{2} ||\theta_i-(\Theta^{t-1}-{h}_i^{t-1})||^2$ is a parameter correction term which regulate the local parameter $\theta_i$ close to drift corrected parameter $\Theta-h_i$, $\alpha$ is a hyper-parameter. In addition, in order to reduce the gradient drift, we add the gradient correction term following the inspiration of Scaffold~\cite{karimireddy2021scaffold},

However, if we optimize the global model parameters directly on the local data set, the inconsistent optimizations on different clients would generate multiple branches of the global model. This is essentially the same as the expected iterative optimization of the global model using the local model in FedAvg.

In FedDC, the parameter drift specifically tracks the deviation between local models and the global model. The three variables are related, so after we update $\theta_i$ to $\theta_i^+$ in each round, we need to update the remaining two variables. First, we introduce the basis for updating $h_i $.
Considering that local training can easily cause model over-fitting, to reduce the influence of local drift to the global model, we decouple the drift to variable $h_i$ that is updated and saved locally.
%In a single client $i$, we convert the optimization goal of the global model $w$ into the optimization goal of the sum of the local model and local drift variables ($\theta_i+h_i$) with $\theta_i$ fixed. 
The local model parameters are the client's prediction of the global parameters. We also denote $\theta_i$ as $w_i$ ($w_i$ represents the global parameters from the perspective of client $i$). Therefore, from the perspective of client $i$, the stage of we update $\theta_i$ to $\theta_i^+$ could be expressed as updating $w_i$ to $w_i^+$ with $\theta_i$ fixed. We can update $h_i$ to $h_i^+$ according to the process shown in Figure \ref{fig_update_h}. That is, $h_i^+=h_i+(w_i^+-w_i)=h_i+(\theta_i^+-\theta_i)$.
\begin{figure}
	\centering
	\includegraphics[width=1\linewidth]{./nips-figs/update_h}
	\caption{The training procedure of FedDC.}
	\label{fig_update_h}
\end{figure}

Then each client participating in the training will correct the local parameters by adding them with the local drift variables and upload the corrected local parameters ($\theta_i^++h_i^+$) to the server. The server performs a weighted average of the corrected local parameters to obtain the global model parameters:
\begin{equation}\label{FedDC_aggragate}
 	w^+= \sum_{i=1}^N \frac{|D_i|}{|D|}(\theta_i^++h_i^+),
\end{equation}
where $|D_i|$ is the sample amount on client $i$, $w^+$ is the updated global model.

\subsection{Training Process}
In the following part, we summarize the training procedure of FedDC with the Expectation-Maximum (EM) algorithm that omits the variable definitions used for transition in the middle, only keeping $h_i$, $\theta_i$ and $w$.. 
The EM algorithm is inspired by the idea of missing data and is used to solve the parameter optimization problem in the case of missing data.  
%Each round of the EM algorithm's optimization procedure is divided into E-step and M-step.
%In E-step, what we do is to fix the value of the model parameters and optimize the distribution of the implicit data. In M-step, what we do is to fix the implicit data according to the data distribution and the optimized values of model parameters.
In federated learning, the hidden information is the implicit global data and model parameters. 
Considering the federated learning algorithm from the perspective of the EM algorithm, on the server-side, we get the local parameters and local drift uploaded by clients, but the training data set and global model parameters are unknown. On the client-side, the known thing is the global model parameters of the last round and the local dataset. We can optimize the local parameters and local drift on the client-side under the premise that the global model parameters are known.

%There are more than one variable in FedDC, so the traditional machine learning method of directly optimizing parameters is not applicable
In FedDC, the traditional machine learning method of directly optimizing parameters is not applicable as there are three types of variables. We can fix two variables to optimize one at a time.  In this way, we seek the extreme value of the other, and finally, approach the extreme value step by step.
Based on the above analysis, we propose to optimize the model in FedDC using the Expectation-Maximum (EM) algorithm. In each round, we execute the Maximization step (M-step) on the client-side to optimize the local parameter and the local drift variables. Then we execute the Expectation step (E-step) on the server-side to update the global parameter. 



\begin{figure}
	\centering
	\includegraphics[width=1\linewidth]{./nips-figs/schedual}
	\caption{The training procedure of FedDC.}
	\label{fig_schedual}
\end{figure}


\begin{algorithm}[htbp]
	\label{algorithmFedDC}
	\small
	\caption{Algorithm of FedDC }
	\KwIn{Random initial global model parameter $w$, set training round $T$, the number of clients $N$, local drift variables $h_i=w-w,\forall i\in [N]$, the learning rate $\eta$, the number of local training batches $K$.}
	\KwOut{The trained global model $w$.}
	%\State some description 
	\For{ $t = 1,2,...,T$}{
		Sample the active client set $C_t\subseteq [N]$.\\ 
		\For{ each client $i \in{C_t}$ in parallel}{
			Set the local model parameter $\theta_i=w,$\\
			\For{ $k = 1,2,...,K$}{ 
				\textbf{Update} the local model parameter: \\$\quad\quad \theta_i=\theta_i+\eta\frac{\partial F(\theta_i|w,h_i,D_i)}{\partial\theta_i}$,
			}
			Set local gradient drift $\Delta\theta_i=\theta_i-w,$\\
			\textbf{Update} the local drift: $ h_i = h_i + \Delta\theta_i,$
		}
		\textbf{Update} the global model: $w=\frac{1}{|C_t|}\sum\limits_{i\in C_t}(\theta_i+h_i),$\\ 
		Set global gradient drift $\Delta \theta=\frac{1}{|C_t|}\sum\limits_{i\in C_t}\Delta\theta_i$,\\
	}
	\textbf{Return} $w$.
\end{algorithm}



The training process of FedDC is shown in Figure \ref{fig_schedual}. 
At M step: our goal is get $\theta_i$ that minimizes Eq. \ref{local_loss} with $w$ and $h_i$ fixed, in each local training iteration, $\theta_i$ is updated by:
\begin{equation}\label{update_theta}
\theta_i=\theta_i+\nabla \theta_i=\theta_i+\eta \frac{\partial{F(\theta_i| w,h_i,D_i)}}{{\partial \theta_i}},
\end{equation}
%\begin{equation}\label{update_theta}
%\theta_i=\arg\min_{\theta_i} F(\theta_i| w,h_i,D_i),
%\end{equation}
then, we fix $w$ and $\theta_i$ to optimize $h_i$ by minimizing the objective function in Eq. \ref{global_loss}, , in each local training iteration, $h_i$ is updated by::
\begin{equation}\label{update_hi}
h_i=hi+\eta\nabla h_i=hi+\eta\frac{\partial{H(h_i| w,\theta_i,D_i)}}{{\partial h_i}},
\end{equation}
at E step: fix $\theta_i$ and $h_i$, optimize $w$; 
\begin{equation}\label{update_w}
w=\sum_{i\in C_t} \frac{|D_i|}{\sum_{i\in C_t}|D_i|}(\theta_i+h_i),
\end{equation}
in this way, we could alternately push the global objective function to the minimum.

%At the begining of each round, active clients download the current global model from the server. Active clients use their own optimizer

To simplify the training process and reduce the computational resource overhead, we reconsider the training process of the local parameters and the local drift variables. We first assume that at the end of each local training round every variable have reached the optimal value under the current known conditions. We suppose $\theta_i$ and $h_i$ are updated to $\theta_i^+$ and $h_i^+$ after this round, suppose $\Delta \theta_i= \theta_i^+-\theta_i, \Delta h_i= h_i^+-h_i$ are their update.
Then we have that:
%$\theta_i^+=\arg\min_{\theta_i} \left\{F(\theta_i| w,h_i,D_i)\right\}$ and $h_i^+=\arg\min_{h_i} \left\{F(h_i| w,\theta_i,D_i)\right\}$.
\begin{equation}\label{update__}
\theta_i^+=\arg\min_{\theta_i} \left\{F(\theta_i| w,h_i,D_i)\right\},
\end{equation}
\begin{equation}\label{update___}
h_i^+=\arg\min_{h_i} \left\{H(h_i| w,\theta_i,D_i)\right\},
\end{equation}
If there are enough local training iterations, with the other two parameters are treated as constants, the above relations always hold regardless of the initial value of the trainable variable.
Expanding Eq. \ref{update__} and Eq. \ref{update___}, then we can easily get that:
$L_i(\theta_i^+) = L_i(\theta_i+h_i^+)=\min(L_i),  ||\theta_i^++h_i-w||^2=0 ,  ||\theta_i+h_i^+-w||^2=0$.
Further, we can derive that if we set the start point of local model parameters as the global model parameter ($\theta_i=w$) at the start of each round while optimizing Eq. \ref{update__}, the following relationship holds: $\Delta h_i=\Delta \theta_i $. This means that we can halve the amount of calclation by setting the start point of $\theta_i$ as $w$ in Eq. \ref{local_loss}. We get the updated value of $h_i$: $h_i^+=h_i+\Delta h_i\approx h_i+\Delta\theta_i$.


Algorithm \ref{algorithmFedDC} shows the workflow of our FedDC. In each training round, the server first selects the active client set. Then the active clients update local model parameters and the corresponding auxiliary drift variables on their local datasets in parallel, and finally, the server aggregates the sum of the local models and drift variables to update the global model.
%FedDC does not directly adopt the average of clients' local parameters as the global parameter. Instead, FedDC decouples the global model and local models with drift variables. 

Although we get multiple personalized local models because of the inevitable heterogeneity issues. In FedDC, the data heterogeneity is reflected in the drift variable, the global model is robust regardless of how much the drift on the client-side.
%At the end of the training, although the local parameters are different from each other, their global parameters reach a consistent global stationary point.

%\subsection{More}
%
%To simplify the training process and reduce the computional resource overhead, we first reconsider the relation of objectives in Equ. \ref and Equ. \ref{}. Observing that the with the local training on objective, we get the updated $h_i+\theta_i$.

%\begin{equation}\label{global_loss}
%w^*= \mathbb{E}_{i\in [N]} (\theta_i+h_i),
%\end{equation}
%
%
%\begin{equation}\label{global_loss}
%w^*=\arg\min_{w} \left\{F(w) = \mathbb{E}_{(x,y)\in D} l(w,(x,y))\right\},
%\end{equation}
%
%\begin{equation}\label{global_loss}
%\theta_i^*=\arg\min_{\theta_i} \left\{F(\theta_i| w,h_i)= \mathbb{E}_{(x,y)\in D_i} l(\theta_i,(x,y))\right\} + ||\theta_i-(w-h_i)||^2,
%\end{equation}
%
%\begin{equation}\label{global_loss}
%h_i^*=\arg\min_{h_i|w,\theta_i} \left\{F(h_i|w,\theta_i)= \mathbb{E}_{(x,y)\in D_i} l((h_i+\theta_i),(x,y))\right\} + ||\theta_i-(w-h_i)||^2,
%\end{equation}

%\subsection{Disscussion}



==> tex_file/analysis.tex <==

\section{Analysis}


\subsection{More Assumption analysis (imitate FedDyn)}
In FLN, each device optimizes its local model to fit its local dataset, recursively. In convergence, the global gradient and local gradients must satisfy that

\begin{equation}\label{1}
\nabla L_c(\Theta)= \nabla L_i(\theta_i)=\nabla L_i(h_i)=0, \quad and \quad \mathbb{E} h_i=\frac{1}{m}\sum_{i=1}^mh_i=0
\end{equation}
where $\Theta_c^t=\Theta_c^{t+1}=\Theta_c^t+\mathbb{E}2 \Delta\Theta^t+\mathbb{E}h_i$, so that $\mathbb{E}h_i=\frac{1}{m}\sum_{i=1}^mh_i=0$.
Set aside the gradient correction term, in $K$ local training iterations that
\begin{equation}\label{2}
\Delta \theta_i^t=\sum_{k=1}^K \nabla_{\theta_i} L_i(\theta_i^{t,k}) = \sum_{k=1}^K \nabla_{\theta_i}\mathbb{E}_{(x,y)\in D_i}l(\theta_i^{t,k},(x,y)) -\alpha \sum_{k=1}^K(\hat{\theta}_i^{t-1}) =0
\end{equation}
that is 
\begin{equation}\label{2}
\sum_{k=1}^K \nabla_{\theta_i}\mathbb{E}_{(x,y)\in D_i}l(\theta_i^{t,k},(x,y)) = \sum_{k=1}^K(\hat{\theta}_i^{t-1})=\alpha K (\Theta^*-h_i^*)
\end{equation}

In FLN, we design the gradient correction term to reduce the instantaneous client-drift, and the regularization term to handle the residual system deviation. 
We build intuition into the two terms of FLN. We note that the system deviation in $t$-th communication round is upper bounded according to Section \ref{}. 
More generally, in $t$-th round, we denote the parameter in client's local model as $\theta_i^t=\theta_i^{t-1}+\Delta \theta_i^t$ and donate the centralized model as $\Theta_c^t=\Theta_c^{t-1}+\Delta \Theta_c^t$. The system diviation of $||\Theta_c^t-\theta_i^t||$
comes from $||\Theta_c^{t-1}-\theta_i^{t-1}||$ which we call residual system diviation and $||\Delta \Theta_c^t -\Delta \theta_i^t||$ which we call the instantaneous client-drift.

\textbf{Gradient correction term.}
\cite{} has proved that the client drift and parameter dissimilarity slowdown FedAVG convergence speed. 
Although the paper \cite{ON THE CONVERGENCE OF FEDAVG ON NON-IID DATA} propose an improved algorithm of FedAVG to make it converge in non-iid datasets. One of their theoretical basis is hypothesis $||\nabla L{(\theta_i^t,D)}-\nabla L{(\theta_i^t,D_i)}||^2\leq \sigma_i^2, \forall i\in [m]$. We analyze below to prove that the value of $\sigma$ is determined by degree of the non-iid data. Taking the cross-entropy loss as example:
\begin{equation}\label{key}
\sigma_i=\nabla_\theta L(\theta_i^t,D)-\nabla_\theta L(\theta_i^t,D_i)=\sum_{c=1}^CP(y=i)\mathbb{E}_{x|y=i}[log f(x,\theta)]-\sum_{c=1}^CP_i(y=i)\mathbb{E}_{x|y=i}[log f(x,\theta)]
\end{equation}
where $P$ is the data distribution of $D$, and $P_i$ is the data distribution of $D_i$. Because the difference between the distributions $P$ and $P_i$ may be arbitrarily different, $\sigma$ is also arbitrarily different.

In FLN, we use the gradient correction term to limit the gradient deviation into a small range that not relies on the data distribution.

%\textbf{$\beta$-smooth Assumption.} 
The global and local objective functions are all $\beta$-smooth: for all $\Theta$ and $\theta$, that satifies:
\begin{equation}\label{key}
||\frac{\partial{L}}{\partial\Theta^{t,k}}-\frac{\partial{L}}{\partial\Theta_i^t}||
<=\beta||\Theta_i^{t,k}-\Theta^t||
\quad and \quad ||\frac{\partial{L_i}}{\partial\theta^{t,k}}-\frac{\partial{L_i}}{\partial\theta_i^t}||
<=\beta||\theta_i^{t,k}-\theta^t||, \quad  \forall i\in[m]
\end{equation}	

Deriving from Equation \ref{lamma1}, the first term of the parameter divation has the upper bounded which is the dunction of $max(||\nabla \theta_f^t-\nabla\theta_i^t||)$, $\forall i \in [N]$. Adding the gradient correction term $\langle\theta_i,\Delta\theta_f^{t-1}-\Delta\theta_i^{t-1 }\rangle$ which makes the update of clients $i$ becomes $\Delta \theta_i^t = g_i(\theta_i)+(\Delta \theta_f^{t-1}-\Delta \theta_i^{t-1}) $. 

%So that the gradient divation is:
%\begin{equation}\label{key}
%||\nabla_\theta L(\theta_i^{t,k},D)-\nabla_\theta L(\theta_i^{t,k},D_i)|| \leq 2\beta||\theta_i^{t,k}-\theta_i^{t-1}||
%\end{equation}
%||(\nabla_\theta L(\theta_t,D)- \nabla_\theta L(\theta_{t-1},D))-(\nabla_\theta L(\theta_t,D_i)-\nabla_\theta L(\theta_{t-1},D_i))||


The difference between the local gradient and the centralized gradient satify that:
\begin{equation}\label{key}
||\frac{\partial{L}}{\partial\theta^{t,k}}- (\frac{\partial{L_i}}{\partial\theta_i^{t,k}}+(\frac{\partial{L}}{\partial\theta^{t}}-\frac{\partial{L_i}}{\partial\theta^{t}}))|| \approx  ||\frac{\partial{L}}{\partial\theta^{t,k}} -(\frac{\partial{L_i}}{\partial\theta_i^{t,k}}
+\frac{1}{K\eta}(\Delta\theta^{t}-\Delta\theta_i^t))||
<=2\beta||\theta_i^{t,k}-\theta^t||
\end{equation}	
where $2\beta||\theta_i^{t,k}-\theta^t||<<\frac{\partial{L}}{\partial\theta^{t,k}}$, so that  the error margin of local gradients to the global gradient is lower bounded regardless their data distribution. 

Under ideal circumstances that neglect communication cost, clients could coorrect its local model each training intertion. As
the corrective lcoal gradients is equivalent to the global gradient, $\frac{\partial{L}}{\partial\theta^{t,k}}\approx (\frac{\partial{L_i}}{\partial\theta_i^{t,k}}+(\frac{\partial{L}}{\partial\theta^{t}}-\frac{\partial{L_i}}{\partial\theta^{t}}))$, it is used to replace the local gradients which with client drifting step by step. However, this not only requires communication too frequent, but also increases the risk of gradient backstepping attacks \cite{}. Adapting the corrective lcoal gradients to federated learning where each communication round catains $K$ local training iteration, we use the $\frac{\partial{L}}{\partial\theta^{t,k}}\approx (\frac{\partial{L_i}}{\partial\theta_i^{t,k}}+\frac{1}{K\eta}(\Delta\theta^{t}-\Delta\theta_i^t))$ to mimic the ideal gradients.



\textbf{regularization term}
Although gradient correction term is used to control client-drift in each local training step, it is inaccurate and the impact of accumulated deviations will gradually increase. We introduce the regularization term to control the accumulated deviations. 

%\textbf{objective inconsistancy}

In addition, the diversity of local data distribution inevitably leads to inconsistent client goals. FedAvg assumes that all clients have the same distribution. Therefore, although the unified global model has considerable average performance, the performance will be greatly reduced on local data sets with the heterogeneous distribution. We denote the model parameters with the best average performance as $\Theta_c^*$, and the best model parameters on the client $i$'s local data set as $\theta_i^*,\forall i\in[m]$. We analyze the reasons for the decrease in FedAvg convergence rate. 

Assuming that the global model of the $t$ round is $\Theta^t$, adopting fixed step-length $a$ optimization, the ideal fixed-length global gradient is $a_g=sign(\Theta_c^*-\Theta^t) a$, that takes $\frac{\Theta_c^*-\Theta^t}{a}$ iterations to converge. In FedAvg, the ideal fixed-length gradient for client $i$ is $a_i=sign(\Theta_t-\theta_i^*)a$, so that the global gradient is $\frac{a_1+a_2}{2}$. Assuming there are two clients, client $1$'s local objective function is $L_1=(\theta-1)^2$, clients $2$'s local objective function is $L_2=(\theta-3)^2$, the global objective function is $L=(\theta-2)^2$.
If $1<\theta<3,\forall theta$, the global gradient is $0$, which means the parameter falls into an area and cannot be optimized to the optimal point $\theta=2$. Even if the fixed-length optimization method is not adopted, in this case, the updates of client $1$ and client $2$ will cancel each other out, resulting in a more minor global update step.

In addition, there are many other factors in federated learning that cause residual system deviation. Updating local parameters and auxiliary deviation variables also helps us resist them and get better global parameters.
Assuming the estimation deviation of clients $i$ in $k$ step of $t$ round in the corrective local gradient and the unbias global gradient is $\sigma^{t,k}$, then the accumulated deviation is as follows:
\begin{equation}\label{key}
\Gamma=\sum_{i=0}^{t-1}\sum_{j=0}^K{\sigma^{i,j}}+\sum_{j=0}^k{\sigma^{t,j}},
\quad where \quad \sigma^{i,j}=||\frac{\partial{L}}{\partial\theta^{t,k}} -(\frac{\partial{L_i}}{\partial\theta_i^{t,k}}
+\frac{1}{K\eta}(\Delta\theta^{t}-\Delta\theta_i^t))||
\end{equation}	


FLN method provides a straightforward way to decople the training accumulated local gradients with model parameter, thus makes up the devition in global parameter.  The previous methods lose the local updating information while local model parameter is simplely replaced with the average of clients' parameters.  FLN keeps local updated information with the optimization state variable $h_i,\quad i\in [m]$, in $t$ round the optimization state variable for clienst $i$ is $h_i^t=\sum_{j=0}^t({\theta_j-\theta_{j-1}})=\sum_{j=0}^t\Delta\theta_{j}$.  

In $t$th round, the cumulative deviation of client $i$'s local model to global model is $\Gamma=h_i^{t}$, where the global state variable $\hat{h}^{t}=\frac{1}{m}\sum_{i=0}^m{h_i^{t}}$. We add an dynamic regularization term in local objective function to fix reduce the cumulative deviation, the regularization term is $\alpha \langle\theta_i,h_i^{t-1} -\Theta^{t-1})\rangle $.  The gap in $t$ round is revised in the following $1/\alpha$ round. The hyperparameter $\alpha$ controls the smoothness of the amendment to prevent a sharp change in gradient wich would damage model performance. 


%无偏估计和有偏估计理论操作之


\textbf{summary}
\cite{} point out that in federated learning, an interplay exists between systems and statistical heterogeneity. If the local dataset of a client has specific data characteristics, it will induce gradients bias in the training process. Inspired by their work, We suggest approximating the ideal gradient based on the current local gradient and the gradient deviation between the local gradients and global gradients in the last round. We update local parameter with the corrective gradients to relieve clients drift. While there are still deviations between the corrective gradients and the truth gradients, we utilize a state variable for each client to hold the optimization state. FLN reduce the cumulative departure between local model and global model to reach precise optimization consistency among clients.


\subsection{Converge Analysis}

==> tex_file/append.tex <==
$\Delta h_i^t =\sum_{i=1}^K \frac{\partial L_i}{\partial h_i^{t,k}} $\\
$\Delta \theta_i^t =\sum_{i=1}^K \frac{\partial L_i}{\partial \theta_i^{t,k}} $\\
$\frac{\partial L_i}{\partial h_i^{t,k}}=\frac{\partial L_i}{\partial \Theta_i^{t,k}}\frac{\partial \Theta_i^{t,k}}{\partial h_i^{t,k}}=\frac{\partial L_i}{\partial \Theta_i^{t,k}}\quad \times 1$\\
$\frac{\partial L_i}{\partial \theta_i^{t,k}}=\frac{\partial L_i}{\partial \Theta_i^{t,k}}\frac{\partial \Theta_i^{t,k}}{\partial \theta_i^{t,k}}=\frac{\partial L_i}{\partial \Theta_i^{t,k}} \quad \times 1$\\
$\frac{\partial L_i}{\partial h_i^{t,k}}=\frac{\partial L_i}{\partial \theta_i^{t,k}}$\\

$L1_i^h=<h,h_i^{t-1}-h_g^{t-1}>$\\
$L2_i^h=<h+\theta,\theta_i^{t-1}+h_g^{t-1}-h_i^{t-1}>=<h,h_g^{t-1}-h_i^{t-1}>$\\$+<h,\theta_i^{t-1}>+<\theta,\theta_i^{t-1}>+<\theta,h_g^{t-1}-h_i^{t-1}>$\\
$\frac{\partial L2_i^h}{\partial \theta}=h_i^{t-1}-h_g^{t-1}=\frac{\partial L1_i^h}{\partial h}$\\



$L(x_t)<L(x_t+h_t)=L(x_t+(h_{t-1}-h_{t-1}^{'}))$\\
$L(x_0)<L(x_0+h_0)$\\
$L(x+h)=L_i(x,h)=\frac{1}{m}\sum_m{L_i(x,h,D_i)}$

Although in this way, clients could remains approximate synchronized gradients, the gradients are inexact. 


Lipschitz smooth
$||\Delta\theta_1-\Delta\theta_2||^2<=L||\theta_1-\theta_2||^2$

$\beta$ smooth
$||\Delta\theta_1-\Delta\theta_2||<=\beta||\theta_1-\theta_2||$

Lipschitz continuous gradient
\begin{equation}
||f^'(x)-f^'(y)<=L||x-y||
\end{equation}
and 
\begin{equation}
f(x)<=f(y)+,\Delta{f(y)}.x-y>+L/2||x-y||^2
\end{equation}
Lipschitz continuous loss
\begin{equation}
||f(x)-f(y)<=L||x-y||
\end{equation}
$f(x)$ is convex function
\begin{equation}
f(y)>=f(x)+f^'(x)(y-x)
\end{equation}
$\mu$ strong convex
$f(x)=\mu/2x^tx$ is convex

quadratic lower bound




With the smooth assumption, we get that $(\Delta\theta_1(D_i)-(\Delta\theta_2(D_i)) <= =\beta||\theta_1-\theta_2|| $. Even though the inexact bias is limited because all varible is updated in each round, the model can not avert a suboptimal because of accumalated bias.   

%Although cumulative deviation correction term is used to control client-side deviation in FedAutoOp, but it is hysteresis and inaccuracy in optimization. We introduce the  gradient correction to further refine our method. 

==> tex_file/checklist.tex <==
\section*{Checklist}
	
	%%% BEGIN INSTRUCTIONS %%%
	The checklist follows the references.  Please
	read the checklist guidelines carefully for information on how to answer these
	questions.  For each question, change the default \answerTODO{} to \answerYes{},
	\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
		justification to your answer}, either by referencing the appropriate section of
	your paper or providing a brief inline description.  For example:
	\begin{itemize}
		\item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
		\item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
		\item Did you include the license to the code and datasets? \answerNA{}
	\end{itemize}
	Please do not modify the questions and only use the provided macros for your
	answers.  Note that the Checklist section does not count towards the page
	limit.  In your paper, please delete this instructions block and only keep the
	Checklist section heading above along with the questions/answers below.
	%%% END INSTRUCTIONS %%%
	
	\begin{enumerate}
		
		\item For all authors...
		\begin{enumerate}
			\item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
			\answerYes{} See Section~\ref{Sec_Intro}.
			\item Did you describe the limitations of your work?
			\answerYes{} See Section~\ref{Sec_exp}.
			\item Did you discuss any potential negative societal impacts of your work?
			\answerNo{} This is a fundamental technical paper.
			\item Have you read the ethics review guidelines and ensured that your paper conforms to them?
			\answerYes{}
		\end{enumerate}
		
		\item If you are including theoretical results...
		\begin{enumerate}
			\item Did you state the full set of assumptions of all theoretical results?
			\answerYes{} See Section~\ref{Sec_method} and Supplemental.
			\item Did you include complete proofs of all theoretical results?
			\answerYes{} See Supplemental.
		\end{enumerate}
		
		\item If you ran experiments...
		\begin{enumerate}
			\item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
			\answerYes{} We include the code in the supplemental material.
			\item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
			\answerYes{} See Section~\ref{Sec_exp}.
			\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
			\answerYes{} See Section~\ref{Sec_exp}.
			\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
			\answerYes{} See Section~\ref{Sec_exp}.
		\end{enumerate}
		
		\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
		\begin{enumerate}
			\item If your work uses existing assets, did you cite the creators?
			\answerYes{} See Section~\ref{Sec_exp}.
			\item Did you mention the license of the assets?
			\answerNo{} We used the public dataset.
			\item Did you include any new assets either in the supplemental material or as a URL?
			\answerNA{}
			\item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
			\answerNA{}
			\item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
			\answerNA{}
		\end{enumerate}
		
		\item If you used crowdsourcing or conducted research with human subjects...
		\begin{enumerate}
			\item Did you include the full text of instructions given to participants and screenshots, if applicable?
			\answerNA{}
			\item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
			\answerNA{}
			\item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
			\answerNA{}
		\end{enumerate}
		
	\end{enumerate}

==> tex_file/method1.tex <==

\subsection{FedAutoOp method.} 
We now present our FedAutoOp method in Algorithm \ref{}. At the begining of each round, active clients download the current global model from the server. Active clients use their own optimizer to minimize their local loss to update their local model. After that, the server aggregates and updates the global model in each round as in FedAVG. 

In heterogeneous client, the optimization direction of the model is not consistent even if they start from the same parameters. In order to track the direction difference, we decouple the optimization of parameters into two parts of the same: parameter optimization and direction optimization. 

\begin{equation}\label{key}
l(\theta)=l(\theta+h), where \hat{\theta}_i^t= \theta_i^{t-1} -\hat{h}_i^t
\end{equation}

where $\theta$ is the model parameter and $h$ is the optimization direction.

In the present FedAutoOp algorithm, the local optimization objective for client $i$ is minizing its local loss which is the sum of its emperical loss on local dataset, its penalized loss term and its gradient correction term:

\begin{equation}\label{key}
\arg \min_{\theta} l_i(\theta+h)= \mathbb{E}_{(x,y)\in D_i}l(\theta+h,(x,y)) - <\theta+h,\theta_{t-1}+(h_{t-1} -\hat(h_{t-1}))>  + <\theta,\Delta\theta_{t-1}-\Delta\theta_{t-1}^g>,
\end{equation}

Keepping the $\theta_0$ fixed, Equation \ref{} is over local pairs $(\theta,h)$. The key technique in the optimization is how to handle this binary optimization problems. We relax the optimization constraints on the parameter $h$ from intertion to round to save computing resources.

Based on Equation \ref{} and Equation \ref{}, we take apart the solution of optimal parameters into a bivariate extreme value solution problem about $\theta$ and $h$. In other works, FedAutoOp method not directly optimize the parameter, but optimize $\theta$ and $h$ to adjust the predicted optimal parameter in each round. Based on the solution process of the extreme value of the binary function, we first get $\frac{L}{\theta}$ according to Equation \ref{}, and then we get $\frac{\partial{L}}{\partial{h}}=\frac{\partial{L}}{\partial{\theta}}\frac{\partial{\theta}}{\partial{h}}$. From Equation \ref{}, $h$ is a variable about $\theta$ and $\frac{\partial{\theta}}{\partial{h}}=-1$ while the $\theta^*$ is a constant, thus $\frac{\partial{L}}{\partial{h}}= \frac{\partial{L}}{\partial{\theta}}$.
Our optimization process will not consume more resources than the standard FedAVG method because we can get $\frac{\partial{L}}{\partial{h}}$ from $\frac{\partial{L}}{\partial{\theta}}$.
  
  
At the end of each round, we set that $\theta=z_t$ as a new starting point for training.  

why need gradient correction term?
\cite{} point out that in federated learning an interplay exists between systems and statistical heterogeneity, that is if the local dataset of a client have specific data characteristics, it will induce gradients bias in the training process. Ispiried by their work, We suggest to count the deviation between the gradients and global gradients from a single client, and add the gradient correction term while calculate its local gradient. 


Why need the regulizer?
In order to unify the optimimal points of heterogeneous clients, we assum that $\hat{h}_i^t$ is the expected gradients bias that makes clinet $i$ optimize towards the consistant minimal $\hat{\theta}^t$. For client $i$, the expected updated parameter in $t$-th round is:
\begin{equation}\label{key}
\hat{\theta}_i^t= \theta_i^{t-1} -\hat{h}_i^t
\end{equation}







==> tex_file/methodnew.tex <==
\section{Method2}

==> tex_file/problem_dinifinition.tex <==
\begin{algorithm}[htbp]
	\caption{FedAVG}
	\KwIn{Initial model parameter $\Theta$, training round $T$, local training iterations $K$, learning rate $\eta$}
	
	\KwOut{The trained global model parameter $\Theta$.}
	%\State some description 
	\For{ $t = 0,1,2,...,T$}{
		Random sample the active clients set $C_t\subseteq [m]$.\\ 
		\For{Client $i \in{C_t}$}{
			initial local model $\theta_i=\Theta$.\\
			Set local objective function $\arg\min\limits_{\theta_i}L_i =  L_{ce}(\theta_i)$.\\
			\For{ $k = 0,1,2,...,K$}{ 
				Update local parameter $\theta_i=\theta_i-\eta\frac{\partial{L_i}}{\partial\theta_i}$\\
			}
		}
		Update global model as $\Theta=\frac{1}{|C_t|}\sum\limits_{i\in C_t}\theta_i$\\
	}
	Return $\Theta$.
\end{algorithm}
\section{Problem Denefinition}

\textbf{Centrelized Learning and Federated Learning.} We first formally define centralized learning and federated learning, then we analyze the difference of their optimizations. 

We assume there are $m$ clients collobarately to train a global model, where each client $i$ owns its local dataset $D_i$. Let $(x,y)$ donates the datapoint, $x$ represents the sample and $y$ is the corresponding ground truth label. In centrelized learning, all data are upload to a server. And the server optimize the following objective function:
\begin{equation}\label{key}
\Theta_c=\arg \min_{\theta}L_c(\theta)= \mathbb{E}_{(x,y)\sim D}l(\theta,(x,y)) = \frac{1}{|D|}\sum_{j=1}^{|D|}l(\theta,(x_{j},y_{j})),
\end{equation}
where $\Theta_c$ is the parameter of centralized learning, $L_c$ is the objective function of centrelized learning, $\theta$ are the model parameters, $D=U\{D_i\}$, $\forall i\in[m]$ is the union dataset of clients' local datasets, $l(\theta,(x,y))$ is the empirimmical loss that measures the distance between the predicted result and the true label. In each training iteration $t$, the parameters in centrelized learning are updated by
\begin{equation}\label{key}
\theta^t=\theta^{t-1}-\eta \nabla_\theta{L_c(\theta^{t-1})}=\theta^{t-1}-\eta \frac{1}{|D|}\sum_{j=1}^{|D|}\nabla_\theta l(\theta^{t-1},(x_{j},y_{j})),
\end{equation}
The server iteratively conducts the SGD optimization to train the model in centralized learning.

Federated learning is a special distributed method that trains models with scattered and privacy data. As the local dataset in federated learning could not be shared, \cite{pmlr-v54-mcmahan17a} designed the FedAVG algorithm. In FedAvg, each clients conduct local SGD optimization steps with its local dataset, respectively. And then server obtains the global model by averaging clients' local models. FedAvg is an approximate solution of Equation \ref{}, in which the global objective function which is the average of clients' local objective functions:
\begin{equation}\label{key}
\Theta_f=\arg \min_{\theta} L_f(\theta)= \frac{1}{m}\sum_{i=1}^m{L_i(\theta)}, \quad  where \quad L_i(\theta)=\mathbb{E}_{(x,y)\sim{D_i}}l(\theta,(x,y)), %= \frac{1}{|D_i|}\sum_{j=1}^{|D_i|}l(\theta,(x_{i,j},y_{i,j}))
\end{equation}
where $\Theta_f$ is the parameter of models in FedAVG, $L_f$ is FedAvg's global objective function, $L_i$ is the local emprimical loss function of client $i$, $\forall i\in [m]$. For ease of expression, we use the average case for their global loss, and it is easy to extend the analysis to weighted-average case. 

In the local optimization phase of FedAvg, each client update its local model with SGD performs in the $k$-th local training iteration of $t$-th communication round:

\begin{equation}\label{key}
\theta_i^{t,k}=\theta_i^{t,k-1}-\eta \nabla_\theta{L_i(\theta_i^{t,k-1})}=\theta_i^{t,k-1}-\eta \frac{1}{|D_i|}\sum_{j=1}^{|D_i|}\nabla_\theta l(\theta_i^{t,k-1},(x_{i,j},y_{i,j})),
\end{equation}


The global optimization process of FedAVG in $t$-th communication round could be simple introduced as follows; each client optimize its local model for $K$ local training iterations starting from the last round's global model. Then the centre server updates clients' global model by averaging the updated local models $\theta^{t,K}=\frac{1}{m}{\theta_i^{t,K}}$. The update value of global model in $t$-th communication round is 

\begin{equation}\label{key}
\theta^{t,K}=\frac{1}{m}\sum_{i=1}^m\theta_i^{t,K}=\theta^{t,0}-\frac{1}{m}\sum_{i=1}^m\sum_{k=1}^K\eta\nabla_\theta{L_i(\theta_i^{t,k-1})}%=\theta_i^{t,0}- \frac{\eta}{m|D_i|}\sum_{i=1}^m\sum_{k=1}^K\sum_{j=1}^{|D_i|}\nabla_\theta l(\theta_i^{t,k-1},(x_{i,j},y_{i,j})),
\end{equation}
where $\theta^{t,0}=\theta^{t-1,K}$ are the parameters of last round's global model. 
 


FedAvg algorithm is the most common used federated learning method. FedAVG utilizes clients' local objective functions as a surrogate to solve the global objective function, making it possible to get an approximate optimal solution. FedAVG reduces communication overhead because it allows the client to run multiple local optimization iterations to minimize its local objectives on the local dataset.  \cite{} provide its converge guarantee with the assumption that local dataset and features are iid. But actually, clients' data are non-iid in most conditions since their local data perhaps collected from diverse backgrounds and devices. Further study \cite{} expand the analysis to the more general condition and found that non-IID data leads clients to inconsistent local updates and inconsistent optimal points. 
In non-iid datasets, FedAVG causes a decrease in the performance of federated learning and slower convergence compared to centralized learning.
We introduce the system deviation between the model parameters of FedAvg and centralized learning below, as it is a crucial notion of this paper. 

\subsection{System Divation}\label{section_client_drift}
\cite{Federated Learning with Non-IID Data}
Denoting the model parameter trained in centralized learning is $\theta^c$, and $\theta^f$ is the model parameter training with FedAVG method in federated learning settings. If there are $m$ clients to jointly solve a $C$ class classification task. For client $i\in[m]$, we assume the data distribution of its local dataset is $P_i$, $P$ is the distribution of centralized union dataset $D=U(D_i)$.

If $\nabla_\theta{l(\theta,(x,y))}$ is $\lambda$-Lipschitz smoothness gradient, we use the cross-entropy loss as empirical loss. In each communication round, clients conduct $K$ steps SGD optimization iterations, the parameter divergence of centralized learning and FedAvg in round $t$ is driven in the following inequality:

\begin{equation}{\label{lamma1}}
\begin{split}
||\theta^f(t,K)-\theta^c(t,K)||&<=\frac{1}{m}\sum_{i=1}^m((\alpha_i)^K||\theta^f(t-1,K)-\theta^c(t-1,K)||\\
&+\eta\frac{1}{m}\sum_{i=1}^m\sum_{j=1}^C||P_i(y=j)-P(y=j)||\sum_{k=0}^{K-1}(\alpha_i)^k\Psi({\theta^c(t,K-1-i)}))
\end{split}
\end{equation}
where $\alpha_i=1+\eta\sum_{j=1}^CP_i(y=j)\lambda{x|y=j}$ and $\Psi(\theta)=max_{j=1}^C||\frac{\partial{l(\theta,(x,y=j))}}{\partial\theta}||$. More detailed proof about Inequality \ref{} is given in Appendix \ref{}.

\textbf{Remark} The parameter divergence between FedAVG and centrelized learning comes from two parts: the parameter divengence of last round $||\theta^f(t-1)-\theta^c(t-1)||$, and the divergence evoked by the difference of data distribution between clients' local datasets and the global dataset, that is $\sum_{j=1}^C||P_i(y=j)-P(y=j)||$. Even if the model start training from the same starting point in centrelized and federated setrtings as $\theta^f(t-1)=\theta^c(t-1)$, the data distribution difference $\sum_{j=1}^C||P_i(y=j)-P(y=j)||$ still leads to parameter differences and reduced accuracy. In addition, an obvious conclusion is that the parameter deviation of each round will be accumulated and amplified while the value $\alpha_i=1+\eta\sum_{j=1}^CP_i(y=j)\lambda{x|y=j}>1$.

\textbf{More parameter deviation from heterogeneity clients.} The parameter deviation not only from non-iid datasets but also from other differences of local optimizations. The clients of federated learning may apply different local learning rates and optimizer, that lead to new inconsistent. In addition, clients could execute different iteration SGD steps in each communication round according to the computing speed of their hardware \cite{wang2020tackling}. \cite{wang2020tackling} show that the global model which is training with heterogeneous local SGD iterations in FedAvg would cause objective inconsistency, and the parameter can be arbitrarily away from the optimal point of the global objective. 
Moreover, accidental training interruption due to network connection and computational constraints also often occurs in the clients of federated learning \cite{}. 
These works demonstrate that the model of federated learning could not reach a periodic consensus point with the model of centralized learning. 

As mentioned above, there are many reasons that cause system deviation. Due to the diversity of deviation reasons and the complexity of their combination, current research only solve one aspect of them. Scaffold \cite{karimireddy2021scaffold} tries to reduce the variance of the local gradients to control the system bias caused by the non-iid data distribution. \cite{NEURIPS2020_564127c0} adjust the weight of parameter aggregation to adapt to the difference in clients' computing speed. \cite{yang2021achieving} explore the impact of only some customers participating in the training on the model. In this article, we use a variable to represent the system deviation regardless of the specific factors that cause the deviation.
%\cite{Federated Learning with Non-IID Data}这个论文有相关的证明，可以拉上来用，我先整理其余部分,SCAFFOLD中也有类似的证明

\subsection{Objective Inconsistency slow down convengecy}
Although the data of different clients are very different, the goal of federated learning is to obtain an efficient global model with the best average performance on the overall data. But the inconsistency of client data leads to the inconsistency of its local target. We give a rational understanding of slow convergence caused by inconsistent goals. We take a quadratic model as the case to tudy the objective inconsistency problem in federated learning. We assum the global objective function is $\arg\min_{w} F(w)=\mathbb{E}_{x\in{D}}\frac{1}{2}||w-x||^2$. If there exist two clients, clien $1$ owns local dataset $D_1$, wher $\mathbb{E}_{x\in{D_1}}x=e_1$; clien $2$ owns local dataset $D_2$, wher $\mathbb{E}_{x\in{D_2}}x=e_2$; and for the global dataset $\mathbb{E}_{x\in{D}}x=\frac{e_1+e_2}{2}$. In FedAvg, if $w_t\in[e_1,e_2]$ then the updates of client $1$ and $2$ have opposite sign, that is they offset each other in the global update.


With the analysis of Section \ref{}, FedAVG \cite{} method optimize the model across different clients by relaxing the equality constraints in $\Theta_c$ and $\Theta_f$ which ignores the system deviation. However, as the analysis, FedAVG can get very different parameters $\Theta_f$ from centralized training parameters $\Theta_c$. We identify that the upper bound of client-drift in a single communication round is not only determined by the degree of clients' non-iid datasets. There are some FedAVG variants like FedProx and SCAFFOLD, which reduce the impact of data heterogeneity by limiting the updates deviation in single-round. However, the FedAVG algorithm and existing variants cannot provably eliminate the system deviation.








==> tex_file/table.tex <==
\begin{table}[!t]\small
	\centering
	\caption{The number of communication round in different methods to achieve a target accuracy while containing with $100$ clients which $100\%$ participating each round. The $SpeedUp$ factor is the number of communication round relative to FedAvg. }
	\label{tab_communication_saving}
	\begin{tabular}{|c|c|cccccc|}
		\hline
		\multirow{2}{*}{Method} &
		\multirow{2}{*}{Accuracy} &
		\multicolumn{2}{c|}{Non-iid (0.6-Dirichlet)} &
		\multicolumn{2}{c|}{Non-iid (0.3-Dirichlet)} &
		\multicolumn{2}{c|}{iid} \\ \cline{3-8} 
		&
		&
		\multicolumn{1}{c|}{Round} &
		\multicolumn{1}{c|}{SpeedUp} &
		\multicolumn{1}{c|}{Round} &
		\multicolumn{1}{c|}{SpeedUp} &
		\multicolumn{1}{c|}{Round} &
		SpeedUp \\ \hline
		\multicolumn{8}{|c|}{CIFAR10 $100$ clients $100\%$ participating} \\ \hline
		\multirow{3}{*}{FedAvg}   & 0.78 & 205 & -       & 346 & -     & 149 & -    \\ \cline{2-2}
		& 0.8  & \textgreater{}1000 & -        & \textgreater{}1000 & -    & 286 & -     \\ \cline{2-2}
		& 0.82 & \textgreater{}1000 & -        & \textgreater{}1000 & -     & 803 & -     \\ \hline
		\multirow{3}{*}{FedProx}  & 0.78 &    195 & 1.05$\times$         & 350    &  0.99$\times$     &   142  &  1.05$\times$     \\ \cline{2-2}
		& 0.8  &  474   &  \textgreater{}2.11$\times$        & \textgreater{}1000    &      1$\times$ &  277   & 1.03$\times$      \\ \cline{2-2}
		& 0.82 &   \textgreater{}1000  &     1$\times$     &   \textgreater{}1000  &    1$\times$   & \textgreater{}1000    &    1$\times$   \\ \hline
		\multirow{3}{*}{Scaffold} &
		0.78$\times$ &		123 &		1.67$\times$ &		148 &		2.34$\times$ &		89 &
		1.67$\times$ \\ \cline{2-2}
		& 0.8  & 165 & >6.06$\times$ & 218 & >4.59$\times$  & 120 & 2.38$\times$  \\ \cline{2-2}
		& 0.82 & 283 & >1.71$\times$ & 387 & >2.58$\times$  & 194 & 4.14$\times$  \\ \hline
		\multirow{3}{*}{FedDyn}   & 0.78 & 44  & 4.66$\times$     & 57  & 6.07$\times$  & 43  & 3.47$\times$  \\ \cline{2-2}
		& 0.8  & 60  & >16.67$\times$    & 75  & >17.54$\times$ & 55  & 5.2$\times$   \\ \cline{2-2}
		& 0.82 & 84  & >11.90$\times$  & 114 & >8.77$\times$  & 75  & 10.7$\times$  \\ \hline
		\multirow{3}{*}{FedDC}     & 0.78 & 43  & 4.77$\times$     & 53  & 6.53$\times$  & 35  & 4.25$\times$  \\ \cline{2-2}
		& 0.8  & 53  & >18.86$\times$  & 70  & >14.28$\times$ & 43  & 6.65$\times$  \\ \cline{2-2}
		& 0.82 & 70  & >14.28$\times$  & 114 & >8.77$\times$  & 56  & 14.34$\times$ \\ \hline\hline
		\multicolumn{8}{|c|}{CIFAR100 $100$ clients $100\%$ participating}               \\ \hline
		\multirow{3}{*}{FedAvg}   & 0.35 & 142 & -        & 112 & -   & 201 & - \\ \cline{2-2}
		& 0.4  & 476 & -      & 847 & -    & \textgreater{}1000 & -    \\ \cline{2-2}
		&
		0.5 &
		\textgreater{}1000 & - &\textgreater{}1000 &	- &		\textgreater{}1000 &		-\\ \hline
		\multirow{3}{*}{FedProx}  &  0.35    & 190    &  0.75$\times$        &  124   &    0.9$\times$   &     145&  1.39$\times$    \\ \cline{2-2}
		&     0.4 & 502    &   0.95$\times$     &  507   &  1.67$\times$     &  273   & >3.66$\times$      \\ \cline{2-2}
		&     0.5 & \textgreater{}1000    &   1$\times$       &   \textgreater{}1000  &  1$\times$     & \textgreater{}1000    &   1$\times$    \\ \hline
		\multirow{3}{*}{Scaffold} & 0.35 & 64  & 2.22$\times$     & 67  & 1.67$\times$  & 58  & 3.47$\times$  \\ \cline{2-2}
		& 0.4  & 91  & >5.23$\times$     & 94  & >9.01$\times$  & 84  & 11.9  \\ \cline{2-2}
		& 0.5  & 424 & >2.35$\times$     & 501 & >2$\times$     & 305 & 3.28$\times$  \\ \hline
		\multirow{3}{*}{FedDyn}   & 0.35 & 38  & 3.74$\times$     & 38  & 2.95$\times$  & 45  & 4.47$\times$  \\ \cline{2-2}
		& 0.4  & 51  & >9.33$\times$     & 53  & >15.98$\times$ & 56  & 17.85$\times$ \\ \cline{2-2}
		& 0.5  & 154 & >6.49$\times$     & 182 & >5.95$\times$  & 169 & 5.92$\times$  \\ \hline
		\multirow{3}{*}{FedDC}     & 0.35 & 30  & 4.73$\times$     & 33  & 3.39$\times$  & 29  & 6.93$\times$  \\ \cline{2-2}
		& 0.4  & 39  & >12.2$\times$     & 41  & >20.65$\times$ & 37  & 27.03$\times$ \\ \cline{2-2}
		& 0.5  & 70  & >14.28$\times$    & 81  & >12.35$\times$ & 70  & 14.28$\times$ \\ \hline
	\end{tabular}
\end{table}



\begin{figure}[!t]
	\centering 
	\subfigbottomskip=2pt
	\subfigcapskip=-5pt 
	\subfigure[]{
		\includegraphics[width=0.3\linewidth]{./nips-figs/F0.15/CIFAR10_100_23_iid_}}
	\subfigure[]{
		\includegraphics[width=0.3\linewidth]{./nips-figs/F0.15/CIFAR100_100_20_Drichlet_0_300}}
	\subfigure[]{
		\includegraphics[width=0.3\linewidth]{./nips-figs/F0.15/CIFAR10_500_23_iid_}}
	\\
	\subfigure[]{
		\includegraphics[width=0.3\linewidth]{./nips-figs/F1.0/CIFAR10_100_23_iid_}}
	%\quad
	\subfigure[]{
		\includegraphics[width=0.3\linewidth]{./nips-figs/F1.0/CIFAR100_100_20_Drichlet_0_300}}
	\subfigure[]{
		\includegraphics[width=0.3\linewidth]{./nips-figs/F1.0/CIFAR100_500_23_iid_}}
	\caption{Convergence plots for FedDC and other baselines in different settings that with $100$ and $500$ clients adopting $100\%$ and $15\%$ client participating settings on iid and non-iid data of CIFAR10 and CIFAR100 datasets.}
\end{figure}\label{figure_converge}



%ACC MNIST EMNIST and Syn CIFAR10 CIFAR100
\begin{table}[!t]\small
	\centering 
	\caption{The convergence accuracy (\%) of models that are trained with different methods (FedDC and the baselines including FedAvg, FedProx, Scaffold and FedDyn) on iid, non-iid and unbalanced data for full (100\%) client participating and part (15\%) participating. We also give the improvements on the accuracy of FedDC compared with FedAvg in the last column. 
	}
	\label{tab-best-accuracy}
	\begin{tabular}{|c|cccccc|}
		\hline
		\multicolumn{1}{|c|}{Data   distribution} &
		\multicolumn{1}{c|}{FedAvg} &
		\multicolumn{1}{c|}{FedProx} &
		\multicolumn{1}{c|}{Scaffold} &
		\multicolumn{1}{c|}{FedDyn} &
		\multicolumn{1}{c|}{FedDC} &
		Improvement \\ \hline\hline
		\multicolumn{7}{|c|}{100 clients 100\% participating}            \\ \hline
		CIFAR10-IID             & 82.16 &81.85 &84.61 & 85.26 & 86.18 & +4.02  \\ %\cline{1-1}
		CIFAR10-Dirichlet(0.3)  & 79.14 &78.89 &82.96 & 84.14 & 84.32 & +5.18  \\ %\cline{1-1}
		CIFAR10-Dirichlet(0.6)  & 80.42 &80.7 &84.13 & 85.26 & 85.64 & +5.22  \\ \cline{1-1}
		CIFAR100-IID            & 39.68 &40.39 &51.26 & 52.07 & 55.52 & +15.84 \\ %\cline{1-1}
		CIFAR100-Dirichlet(0.3) & 40.11 &40.93 &50.44 & 51.89 & 54.86 & +14.75 \\ %\cline{1-1}
		CIFAR100-Dirichlet(0.6) & 40.48 &40.15 &51.16 & 52.84 & 55.34 & +14.86 \\ \hline\hline
		\multicolumn{7}{|c|}{100 clients 15\% participating}            \\ \hline
		CIFAR10-IID             & 81.67 &82.16 &84.68 & 84.5  & 85.71 & +4.04  \\ 
		CIFAR10-Dirichlet(0.3)  & 79.77  &79.84 &82.53  &  82.3  & 84.58  & +4.81  \\	%\cline{1-1}
		CIFAR10-Dirichlet(0.6)  & 81.05 &81.32 &83.57 & 84.1  & 84.77 & +3.72  \\ \cline{1-1}
		CIFAR100-IID            & 40.8  &40.67 &49.8  & 51.2  & 55.4  & +14.6  \\ 
		CIFAR100-Dirichlet(0.3) & 41.81  &41.84 &50.25  & 51.13   & 53.91  & +4.1   \\ %\cline{1-1}
		CIFAR100-Dirichlet(0.6) & 41.76 &41.83 &50.01 & 51.75 & 54.65 & +12.89 \\ \hline\hline
		\multicolumn{7}{|c|}{500 clients 100\% participating}            \\ \hline
		CIFAR10-IID             & 73.43 &72.77 &81.56 & 84.07 & 84.93 & +11.5  \\ \cline{1-1}
		CIFAR100-IID            & 26.03 &28.22 &45.62 & 50.22 & 54.25 & +28.22 \\ \hline\hline
		\multicolumn{7}{|c|}{500 clients 15\% participating}            \\ \hline
		CIFAR10-IID             & 73.26 &72.58 &81.58 & 82.49 & 84.19 & +10.93 \\ \cline{1-1}
		CIFAR100-IID            & 27.36 & 26.5 &30.45 & 44.11 & 50.61 & +23.25 \\ \hline \hline
		\multicolumn{7}{|c|}{100 clients 100\% participating}            \\ \hline
		CIFAR10-unbalance             & 81.37 &81.9 &84.45 & 85.68 & 86.31 &  +4.94\\ \cline{1-1}
		CIFAR100-unbalance            & 40.03 &39.93 &51.3 & 52.81 & 55.69 & +15.66 \\ \hline
		\multicolumn{7}{|c|}{100 clients 15\% participating}            \\ \hline
		CIFAR10-unbalance             & 81.68 & 81.88 &84.44 & 84.3 & 85.35 &  +3.67\\ \cline{1-1}
		CIFAR100-unbalance            & 40.9 &41.05 &50.57 & 51.01 & 55.27 & +14.35 \\ \hline\hline
		\multicolumn{7}{|c|}{100 clients 100\% participating}            \\ \hline
		MNIST-IID             & 98.12  & 98.12   & 98.32    & 98.51  & 98.45 & +0.33  \\ %\cline{1-1}
		MNIST-Dirichlet(0.3)   & 97.98  & 97.96   & 98.45    & 98.46  & 98.51 &  +0.53  \\ %\cline{1-1}
		MNIST-Dirichlet(0.6)   & 98.09  & 98.05   & 98.39    & 98.44  & 98.48 &  +0.39  \\
		MNIST-Unbalance    & 98.12  & 98.1    & 98.35    & 98.6   & 98.46 &  +0.34  \\ \cline{1-1}
		EMNIST-L-IID            & 94.82  & 94.66   & 95.64    & 95.3   & 95.55 &  +0.73 \\ %\cline{1-1}
		EMNIST-L-Dirichlet(0.3)  & 94.34  & 94.3    & 95.36    & 94.99  & 95.27 &  +0.93     \\ %\cline{1-1}
		EMNIST-L-Dirichlet(0.6) & 94.38  & 94.48   & 95.51    & 95.34  & 95.46 &  +1.08   \\ \hline\hline
		\multicolumn{7}{|c|}{100 clients 15\% participating}            \\ \hline
		MNIST-IID             & 98.15 & 98.11 & 98.45 & 98.38 & 98.47 &  +0.32  \\ 
		MNIST-Dirichlet(0.3)  & 98    & 98.04 & 98.37 & 98.3  & 98.4  &  +0.4   \\	%\cline{1-1}
		MNIST-Dirichlet(0.6)  & 98.13 & 98.12 & 98.49 & 98.3  & 98.49 &  +0.36  \\ 
		MNIST-Unbalance  	 & 98.15 & 98.13 & 98.5  & 98.34 & 98.5  &  +0.35  \\ \cline{1-1}
		EMNIST-L-IID            & 94.83 & 94.67 & 95.44 & 95.23 & 95.71 &  +0.88   \\ 
		EMNIST-L-Dirichlet(0.3) & 94.05 & 94.13 & 95.05 & 94.58 & 95    &  +0.95   \\ %\cline{1-1}
		EMNIST-L-Dirichlet(0.6) & 94.39 & 94.37 & 95.53 & 94.93 & 95.42 &  +1.03  \\ \hline\hline
		\multicolumn{7}{|c|}{100 clients 100\% participating}            \\ \hline
		Syn(0,0)              & 98.65 & 98.65 & 98.65 & 99.25 & 99.35 &  +0.7 \\ 
		Syn(1,0)             & 97.83 & 97.82 & 97.9  & 98.65 & 98.83 &  +1     \\ 
		Syn(0,1)             & 97.75 & 97.75 & 97.9  & 99.1  & 99.3  &  +1.55 \\ \hline
		\multicolumn{7}{|c|}{100 clients 15\% participating}            \\ \hline
		Syn(0,0)             & 98.75 & 98.7  & 98.65 & 99.32 & 99.57 &  +0.82\\ 
		Syn(1,0)            & 97.7  & 97.67 & 97.9  & 98.82 & 99.23 &  +1.53   \\ 
		Syn(0,1)             & 98.52 & 98.5  & 98.58 & 99.3  & 99.62 &  +1.1 \\ \hline
	\end{tabular}
\end{table}




\begin{table}[!t]\small
	\centering
	\caption{The number of communication round in different methods to achieve a target accuracy on CIFAR10 and CIFAR100 while containing with $100$ clients which $100\%$ participating each round. The $SpeedUp$ factor is the number of communication round relative to FedAvg. }
	\label{tab_communication_saving}
	\begin{tabular}{|c|c|cccccc|}
		\hline
		\multirow{2}{*}{Method} &
		\multirow{2}{*}{Accuracy} &
		\multicolumn{2}{c|}{Non-iid (0.6-Dirichlet)} &
		\multicolumn{2}{c|}{Non-iid (0.3-Dirichlet)} &
		\multicolumn{2}{c|}{iid} \\ \cline{3-8} 
		&
		&
		\multicolumn{1}{c|}{Round} &
		\multicolumn{1}{c|}{SpeedUp} &
		\multicolumn{1}{c|}{Round} &
		\multicolumn{1}{c|}{SpeedUp} &
		\multicolumn{1}{c|}{Round} &
		SpeedUp \\ \hline
		\multicolumn{8}{|c|}{CIFAR10 $100$ clients $100\%$ participating} \\ \hline
		\multirow{3}{*}{FedAvg}   & 0.78 & 205 & -       & 346 & -     & 149 & -    \\ \cline{2-2}
		& 0.8  & \textgreater{}1000 & -        & \textgreater{}1000 & -    & 286 & -     \\ \cline{2-2}
		& 0.82 & \textgreater{}1000 & -        & \textgreater{}1000 & -     & 803 & -     \\ \hline
		\multirow{3}{*}{FedProx}  & 0.78 &    195 & 1.05$\times$         & 350    &  0.99$\times$     &   142  &  1.05$\times$     \\ \cline{2-2}
		& 0.8  &  474   &  \textgreater{}2.11$\times$        & \textgreater{}1000    &      1$\times$ &  277   & 1.03$\times$      \\ \cline{2-2}
		& 0.82 &   \textgreater{}1000  &     1$\times$     &   \textgreater{}1000  &    1$\times$   & \textgreater{}1000    &    1$\times$   \\ \hline
		\multirow{3}{*}{Scaffold} &
		0.78$\times$ &		123 &		1.67$\times$ &		148 &		2.34$\times$ &		89 &
		1.67$\times$ \\ \cline{2-2}
		& 0.8  & 165 & >6.06$\times$ & 218 & >4.59$\times$  & 120 & 2.38$\times$  \\ \cline{2-2}
		& 0.82 & 283 & >1.71$\times$ & 387 & >2.58$\times$  & 194 & 4.14$\times$  \\ \hline
		\multirow{3}{*}{FedDyn}   & 0.78 & 44  & 4.66$\times$     & 57  & 6.07$\times$  & 43  & 3.47$\times$  \\ \cline{2-2}
		& 0.8  & 60  & >16.67$\times$    & 75  & >17.54$\times$ & 55  & 5.2$\times$   \\ \cline{2-2}
		& 0.82 & 84  & >11.90$\times$  & 114 & >8.77$\times$  & 75  & 10.7$\times$  \\ \hline
		\multirow{3}{*}{FedDC}     & 0.78 & 43  & 4.77$\times$     & 53  & 6.53$\times$  & 35  & 4.25$\times$  \\ \cline{2-2}
		& 0.8  & 53  & >18.86$\times$  & 70  & >14.28$\times$ & 43  & 6.65$\times$  \\ \cline{2-2}
		& 0.82 & 70  & >14.28$\times$  & 114 & >8.77$\times$  & 56  & 14.34$\times$ \\ \hline\hline
		\multicolumn{8}{|c|}{CIFAR100 $100$ clients $100\%$ participating}               \\ \hline
		\multirow{3}{*}{FedAvg}   & 0.35 & 142 & -        & 112 & -   & 201 & - \\ \cline{2-2}
		& 0.4  & 476 & -      & 847 & -    & \textgreater{}1000 & -    \\ \cline{2-2}
		&
		0.5 &
		\textgreater{}1000 & - &\textgreater{}1000 &	- &		\textgreater{}1000 &		-\\ \hline
		\multirow{3}{*}{FedProx}  &  0.35    & 190    &  0.75$\times$        &  124   &    0.9$\times$   &     145&  1.39$\times$    \\ \cline{2-2}
		&     0.4 & 502    &   0.95$\times$     &  507   &  1.67$\times$     &  273   & >3.66$\times$      \\ \cline{2-2}
		&     0.5 & \textgreater{}1000    &   1$\times$       &   \textgreater{}1000  &  1$\times$     & \textgreater{}1000    &   1$\times$    \\ \hline
		\multirow{3}{*}{Scaffold} & 0.35 & 64  & 2.22$\times$     & 67  & 1.67$\times$  & 58  & 3.47$\times$  \\ \cline{2-2}
		& 0.4  & 91  & >5.23$\times$     & 94  & >9.01$\times$  & 84  & 11.9  \\ \cline{2-2}
		& 0.5  & 424 & >2.35$\times$     & 501 & >2$\times$     & 305 & 3.28$\times$  \\ \hline
		\multirow{3}{*}{FedDyn}   & 0.35 & 38  & 3.74$\times$     & 38  & 2.95$\times$  & 45  & 4.47$\times$  \\ \cline{2-2}
		& 0.4  & 51  & >9.33$\times$     & 53  & >15.98$\times$ & 56  & 17.85$\times$ \\ \cline{2-2}
		& 0.5  & 154 & >6.49$\times$     & 182 & >5.95$\times$  & 169 & 5.92$\times$  \\ \hline
		\multirow{3}{*}{FedDC}     & 0.35 & 30  & 4.73$\times$     & 33  & 3.39$\times$  & 29  & 6.93$\times$  \\ \cline{2-2}
		& 0.4  & 39  & >12.2$\times$     & 41  & >20.65$\times$ & 37  & 27.03$\times$ \\ \cline{2-2}
		& 0.5  & 70  & >14.28$\times$    & 81  & >12.35$\times$ & 70  & 14.28$\times$ \\ \hline
	\end{tabular}
\end{table}




\begin{table}[!t]\small
	\centering
	\caption{The number of communication round in different methods to achieve a target accuracy while containing with $100$ clients which $15\%$ participating each round. The $SpeedUp$ factor is the number of communication round relative to FedAvg.}
	\label{tab_communication_saving_15}
	\begin{tabular}{|c|c|cccccc|}
		\hline
		\multirow{2}{*}{Method} &
		\multirow{2}{*}{Accuracy} &
		\multicolumn{2}{c|}{Non-iid (0.6-Dirichlet)} &
		\multicolumn{2}{c|}{Non-iid (0.3-Dirichlet)} &
		\multicolumn{2}{c|}{iid} \\ \cline{3-8} 
		&
		&
		\multicolumn{1}{c|}{Round} &
		\multicolumn{1}{c|}{SpeedUp} &
		\multicolumn{1}{c|}{Round} &
		\multicolumn{1}{c|}{SpeedUp} &
		\multicolumn{1}{c|}{Round} &
		SpeedUp \\ \hline
		\multicolumn{8}{|c|}{CIFAR10 $100$ clients $15\%$ participating} \\ \hline
		\multirow{3}{*}{FedAvg}   & 0.78 & 259 & -       & 491 & -     & 177 & -     \\ \cline{2-2}
		& 0.8  &616 & -        & \textgreater{}1000 & -     & \textgreater{}1000 & -     \\ \cline{2-2}
		& 0.82 & \textgreater{}1000 & -        & \textgreater{}1000 & -    &\textgreater{}1000 & -     \\ \hline
		\multirow{3}{*}{FedProx}  & 0.78   &  228        &1.13$\times$     & 485      &  1.1$\times$   &153& 1.15$\times$      \\ \cline{2-2}
		& 0.8  &  459   & 1.34$\times$         &  \textgreater{}1000   &   1$\times$  &  307   &    \textgreater{}3.28   \\ \cline{2-2}
		& 0.82 &  \textgreater{}1000   &     1$\times$     &   \textgreater{}1000  &    1$\times$   &   \textgreater{}1000  &     1$\times$ \\ \hline
		\multirow{3}{*}{Scaffold} &
		0.78&
		132 &
		1.96$\times$ &
		169 &
		2.91$\times$ &
		94 &
		1.88$\times$ \\ \cline{2-2}
		& 0.8  & 200 & 3.08$\times$ & 263 & >3.80$\times$  & 126 & >7.93$\times$  \\ \cline{2-2}
		& 0.82 & 332 & >3.01$\times$ & 600 & >1.67$\times$  & 204 & >4.9$\times$  \\ \hline
		\multirow{3}{*}{FedDyn}   & 0.78 & 118  & 2.19$\times$     & 146  & 3.39$\times$  & 110  & 1.61$\times$  \\ \cline{2-2}
		& 0.8  & 193  & 3.19$\times$    & 195  & >5.12$\times$ & 145  & >6.9$\times$   \\ \cline{2-2}
		& 0.82 & 254 & >3.93$\times$  & 512 & >1.95$\times$  & 231  & >4.33$\times$  \\ \hline
		\multirow{3}{*}{FedDC}     & 0.78 & 101  & 2.56$\times$     & 105  & 4.68$\times$  & 88  & 2.01$\times$  \\ \cline{2-2}
		& 0.8  & 141  & 4.37$\times$  & 143  & >6.99$\times$ & 108  & >9.26$\times$  \\ \cline{2-2}
		& 0.82 & 211  & >4.74$\times$  & 242 & >4.13$\times$  & 162  & >6.17$\times$ \\ \hline\hline
		\multicolumn{8}{|c|}{CIFAR100 $100$ clients $15\%$ participating}               \\ \hline
		\multirow{3}{*}{FedAvg}   & 0.35 & 170 & -       & 144 & -    & 260 & -     \\ \cline{2-2}
		& 0.4  & 615 & -        & 520 & -     & 724 & -    \\ \cline{2-2}
		&
		0.5 &
		\textgreater{}1000 &- &\textgreater{}1000 &	- &		\textgreater{}1000 &		- \\ \hline
		\multirow{3}{*}{FedProx}  &  0.35    & 227    &  0.75$\times$        &   148  &  0.97$\times$     &  187   &   1.39$\times$    \\ \cline{2-2}
		&    0.4  &    980 &    0.63$\times$      &  503   &    1.03$\times$   & 650    &    >1.11$\times$   \\ \cline{2-2}
		&     0.5 &   >1000  &    1$\times$      &  >1000   &    1$\times$   &   >1000  &     1$\times$  \\ \hline
		\multirow{3}{*}{Scaffold} & 0.35 & 68  & 2.5$\times$     & 72  & 2$\times$  & 68 & 3.82$\times$  \\ \cline{2-2}
		& 0.4  & 106  & 5.8$\times$     & 114  & 3.56$\times$  & 113  & 6.41$\times$  \\ \cline{2-2}
		& 0.5  & >1000 & 1$\times$     & >1000 & 1$\times$    & >1000 & 1$\times$ \\ \hline
		\multirow{3}{*}{FedDyn}   & 0.35 & 98  & 1.73$\times$     & 78  & 1.46$\times$  & 106  & 2.45$\times$  \\ \cline{2-2}
		& 0.4  & 149  & 4.42$\times$     & 148  & 3.51$\times$ & 143  & 5.06$\times$ \\ \cline{2-2}
		& 0.5  & 574 & >1.74$\times$     & 710 & >1.41$\times$  & 619 & 1.62$\times$  \\ \hline
		\multirow{3}{*}{FedDC}     & 0.35 & 78  & 2.18$\times$     & 74  & 1.54$\times$  & 74  & 3.51$\times$  \\ \cline{2-2}
		& 0.4  & 102  & 6.03$\times$     & 103  & 5.05$\times$ & 100  & 7.04$\times$ \\ \cline{2-2}
		& 0.5  & 249  & >4.02$\times$    & 278  & >3.6$\times$ & 206  & >4.85$\times$ \\ \hline
	\end{tabular}
\end{table}

\begin{table}[!t]\small
	\centering
	\caption{The number of communication round in different methods to achieve a target accuracy on MNIST and EMNIST-L while containing with $100$ clients which $100\%$ participating each round. The $SpeedUp$ factor is the number of communication round relative to FedAvg. }
	\label{tab_communication_saving}
	\begin{tabular}{|c|c|cccccc|}
		\hline
		\multirow{2}{*}{Method} &
		\multirow{2}{*}{Accuracy} &
		\multicolumn{2}{c|}{Non-iid (0.6-Dirichlet)} &
		\multicolumn{2}{c|}{Non-iid (0.3-Dirichlet)} &
		\multicolumn{2}{c|}{iid} \\ \cline{3-8} 
		&
		&
		\multicolumn{1}{c|}{Round} &
		\multicolumn{1}{c|}{SpeedUp} &
		\multicolumn{1}{c|}{Round} &
		\multicolumn{1}{c|}{SpeedUp} &
		\multicolumn{1}{c|}{Round} &
		SpeedUp \\ \hline
		\multicolumn{8}{|c|}{MNIST $100$ clients $100\%$ participating} \\ \hline
		\multirow{2}{*}{FedAvg}   & 0.96        & 25                &-      & 28                &-       & 16                & -           \\ \cline{2-2}
		& 0.98  & 258               & -     & 492               &-          & 142               & -            \\ \hline
		\multirow{2}{*}{FedProx}   & 0.96      & 24                & 1.04$\times$       & 27                & 1.04$\times$& 16                & 1$\times$   \\ \cline{2-2}
		& 0.98  & 263               & 0.98$\times$  & 480               & 1.03$\times$        & 136               & 1.04$\times$ \\ \hline
		\multirow{2}{*}{Scaffold} 
		& 0.96   & 11                & 2.27$\times$ & 14                & 2$\times$            & 9                 & 1.78$\times$\\ \cline{2-2}
		& 0.98  & 58                & 4.45$\times$ & 58                & 8.48$\times$  & 53                & 2.68$\times$\\ \hline
		\multirow{2}{*}{FedDyn}  & 0.96& 8                 & 3.13$\times$   & 9                 & 3.11$\times$  & 7                 & 2.29$\times$   \\ \cline{2-2}
		& 0.98  & 46                & 5.61$\times$& 51                & 9.65$\times$  & 27                & 5.26$\times$\\ \hline
		\multirow{2}{*}{FedDC}     & 0.96 & 8                 & 3.13$\times$ & 10                & 2.8$\times$         & 7                 & 2.29$\times$ \\ \cline{2-2}
		& 0.98   & 35                & 7.37$\times$& 37                & 13.3$\times$ & 26                & 5.46$\times$\\ \hline\hline
		\multicolumn{8}{|c|}{EMNIST-L $100$ clients $100\%$ participating}               \\ \hline
		\multirow{2}{*}{FedAvg}    & 0.94  & 142               &-  & 192               & -          & 107               & -            \\ \cline{2-2}
		& 0.95 & \textgreater{}300 & -           & \textgreater{}300 & -           & \textgreater{}300 &- \\ \hline
		\multirow{2}{*}{FedProx}  & 0.94& 135               & 1.05$\times$  & 198               & 0.97$\times$    & 92                & 1.16$\times$ \\ \cline{2-2}
		& 0.95 & \textgreater{}300 & 1$\times$           & \textgreater{}300 & 1$\times$           & \textgreater{}300 & 1$\times$      \\ \hline
		\multirow{3}{*}{Scaffold}  & 0.94 & 43                & 3.30$\times$& 52                & 3.69$\times$  & 30                & 3.57$\times$ \\ \cline{2-2}
		& 0.95  & 75                & \textgreater{}4$\times$    & 150               & \textgreater{}2$\times$              & 66                &\textgreater{} 4.55$\times$   \\ \hline
		\multirow{2}{*}{FedDyn}    & 0.94 & 30                & 4.73$\times$  & 52                & 3.69$\times$  & 27                & 3.96$\times$\\ \cline{2-2}
		& 0.95  & 137               & \textgreater{}2.19$\times$& 160               & \textgreater{}1.88$\times$          & 69                & \textgreater{}4.35$\times$\\ \hline
		\multirow{2}{*}{FedDC}      & 0.94  & 43                & 3.3$\times$ & 60                & 3.2$\times$          & 21                & 5.1$\times$ \\ \cline{2-2}
		& 0.95      & 78                & \textgreater{}3.85$\times$    & 134               & \textgreater{}2.24$\times$   & 50                & \textgreater{}6$\times$  \\ \hline
	\end{tabular}
\end{table}

\begin{table}[!t]\small
	\centering
	\caption{The number of communication round in different methods to achieve a target accuracy on MNIST and EMNIST-L while containing with $100$ clients which $15\%$ participating each round. The $SpeedUp$ factor is the number of communication round relative to FedAvg. }
	\label{tab_communication_saving}
	\begin{tabular}{|c|c|cccccc|}
		\hline
		\multirow{2}{*}{Method} &
		\multirow{2}{*}{Accuracy} &
		\multicolumn{2}{c|}{Non-iid (0.6-Dirichlet)} &
		\multicolumn{2}{c|}{Non-iid (0.3-Dirichlet)} &
		\multicolumn{2}{c|}{iid} \\ \cline{3-8} 
		&
		&
		\multicolumn{1}{c|}{Round} &
		\multicolumn{1}{c|}{SpeedUp} &
		\multicolumn{1}{c|}{Round} &
		\multicolumn{1}{c|}{SpeedUp} &
		\multicolumn{1}{c|}{Round} &
		SpeedUp \\ \hline
		\multicolumn{8}{|c|}{MNIST $100$ clients $15\%$ participating} \\ \hline
		\multirow{2}{*}{FedAvg}  & 0.96      & 32                & -      & 35                & -         & 23                & -     \\ \cline{2-2}
		& 0.98     & 361               & -     & \textgreater{}600 & -         & 158               & -              \\ \hline
		\multirow{2}{*}{FedProx}  & 0.96      & 31                & 1.03$\times$     & 34                & 1.03$\times$  & 23                & 1$\times$ \\ \cline{2-2}
		& 0.98 & 383               & 0.94$\times$ & 418               & \textgreater{}1.44$\times$  & 149               & 1.06$\times$\\ \hline
		\multirow{2}{*}{Scaffold} 
		& 0.96    & 20                & 1.6$\times$  & 23                & 1.52$\times$     & 16                & 1.44$\times$   \\ \cline{2-2}
		& 0.98    & 62                & 5.82$\times$     & 72                &\textgreater{} 8.33$\times$  & 50                & 3.16$\times$  \\ \hline
		\multirow{2}{*}{FedDyn}   & 0.96 & 21                & 1.52$\times$ & 23                & 1.52$\times$    & 18                & 1.28$\times$ \\ \cline{2-2}
		& 0.98  & 122               & 2.96$\times$ & 153               & \textgreater{}3.92$\times$ & 71                & 2.23$\times$ \\ \hline
		\multirow{2}{*}{FedDC}      & 0.96   & 18                & 1.78$\times$     & 22                & 1.59$\times$  & 16                & 1.44$\times$ \\ \cline{2-2}
		& 0.98  & 60      & 6.02$\times$ & 62                &\textgreater{} 9.68$\times$           & 46                & 3.43$\times$ \\ \hline\hline
		\multicolumn{8}{|c|}{EMNIST-L $100$ clients $15\%$ participating}               \\ \hline
		\multirow{2}{*}{FedAvg}    & 0.94   & 153               & -       & 245               &-           & 108               & -          \\ \cline{2-2}
		& 0.95 & \textgreater{}300 & -           & \textgreater{}300 & -           & \textgreater{}300 & -     \\ \hline
		\multirow{2}{*}{FedProx}  & 0.94  & 145               & 1.06$\times$  & 240               & 1.02$\times$   & 105               & 1.03$\times$ \\ \cline{2-2}
		& 0.95 & \textgreater{}300 & 1$\times$           & \textgreater{}300 & 1$\times$           & \textgreater{}300 & 1$\times$        \\ \hline
		\multirow{3}{*}{Scaffold} & 0.94   & 44                & 3.48$\times$ & 68                & 3.6$\times$& 42                & 2.57$\times$\\ \cline{2-2}
		& 0.95 & 95                & \textgreater{}4.21$\times$  & \textgreater{}300 & 1$\times$           & 87                & \textgreater{}3.45$\times$  \\ \hline
		\multirow{2}{*}{FedDyn}     & 0.94& 73                & 2.1$\times$  & 81                & 3.06$\times$        & 61                & 1.61$\times$  \\ \cline{2-2}
		& 0.95    & 127               & \textgreater{}2.36$\times$ & \textgreater{}300 & 1$\times$          & 255               & \textgreater{}1.18$\times$\\ \hline
		\multirow{2}{*}{FedDC}      & 0.94  & 48                & 3.19$\times$  & 74                & 3.31$\times$ & 47                & 2.3$\times$    \\ \cline{2-2}
		& 0.95 & 92                & \textgreater{}3.26$\times$ & \textgreater{}300 & 1$\times$           & 81                & \textgreater{}3.7$\times$ \\ \hline
	\end{tabular}
\end{table}

\begin{table}[!t]\small
	\centering 
	\caption{The convergence accuracy (\%) of models that are trained with different methods (FedDC and three baselines including FedAvg, Scaffold and FedDyn) on iid, non-iid and unbalanced data for full (100\%) client participating and part (15\%) participating. We also give the improvements on the accuracy of FedDC compared with FedAvg in the last column. 
	}
	\label{tab-best-accuracy}
	\begin{tabular}{|c|cccccc|}
		\hline
		\multicolumn{1}{|c|}{Data   distribution} &
		\multicolumn{1}{c|}{FedAvg} &
		\multicolumn{1}{c|}{FedProx} &
		\multicolumn{1}{c|}{Scaffold} &
		\multicolumn{1}{c|}{FedDyn} &
		\multicolumn{1}{c|}{FedDC} &
		Improvement \\ \hline\hline
		\multicolumn{7}{|c|}{100 clients 100\% participating}            \\ \hline
		CIFAR10-IID             & 82.16 &81.85 &84.61 & 85.26 & 86.18 & +4.02  \\ %\cline{1-1}
		CIFAR10-Dirichlet(0.3)  & 79.14 &78.89 &82.96 & 84.14 & 84.32 & +5.18  \\ %\cline{1-1}
		CIFAR10-Dirichlet(0.6)  & 80.42 &80.7 &84.13 & 85.26 & 85.64 & +5.22  \\ \cline{1-1}
		CIFAR100-IID            & 39.68 &40.39 &51.26 & 52.07 & 55.52 & +15.84 \\ %\cline{1-1}
		CIFAR100-Dirichlet(0.3) & 40.11 &40.93 &50.44 & 51.89 & 54.86 & +14.75 \\ %\cline{1-1}
		CIFAR100-Dirichlet(0.6) & 40.48 &40.15 &51.16 & 52.84 & 55.34 & +14.86 \\ \hline\hline
		\multicolumn{7}{|c|}{100 clients 15\% participating}            \\ \hline
		CIFAR10-IID             & 81.67 &82.16 &84.68 & 84.5  & 85.71 & +4.04  \\ 
		CIFAR10-Dirichlet(0.3)  & 79.77  &79.84 &82.53  &  82.3  & 84.58  & +4.81  \\	%\cline{1-1}
		CIFAR10-Dirichlet(0.6)  & 81.05 &81.32 &83.57 & 84.1  & 84.77 & +3.72  \\ \cline{1-1}
		CIFAR100-IID            & 40.8  &40.67 &49.8  & 51.2  & 55.4  & +14.6  \\ 
		CIFAR100-Dirichlet(0.3) & 41.81  &41.84 &50.25  & 51.13   & 53.91  & +4.1   \\ %\cline{1-1}
		CIFAR100-Dirichlet(0.6) & 41.76 &41.83 &50.01 & 51.75 & 54.65 & +12.89 \\ \hline\hline
		\multicolumn{7}{|c|}{500 clients 100\% participating}            \\ \hline
		CIFAR10-IID             & 73.43 &72.77 &81.56 & 84.07 & 84.93 & +11.5  \\ \cline{1-1}
		CIFAR100-IID            & 26.03 &28.22 &45.62 & 50.22 & 54.25 & +28.22 \\ \hline\hline
		\multicolumn{7}{|c|}{500 clients 15\% participating}            \\ \hline
		CIFAR10-IID             & 73.26 &72.58 &81.58 & 82.49 & 84.19 & +10.93 \\ \cline{1-1}
		CIFAR100-IID            & 27.36 & 26.5 &30.45 & 44.11 & 50.61 & +23.25 \\ \hline \hline
		\multicolumn{7}{|c|}{100 clients 100\% participating}            \\ \hline
		CIFAR10-unbalance             & 81.37 &81.9 &84.45 & 85.68 & 86.31 &  +4.94\\ \cline{1-1}
		CIFAR100-unbalance            & 40.03 &39.93 &51.3 & 52.81 & 55.69 & +15.66 \\ \hline
		\multicolumn{7}{|c|}{100 clients 15\% participating}            \\ \hline
		CIFAR10-unbalance             & 81.68 & 81.88 &84.44 & 84.3 & 85.35 &  +3.67\\ \cline{1-1}
		CIFAR100-unbalance            & 40.9 &41.05 &50.57 & 51.01 & 55.27 & +14.35 \\ \hline
	\end{tabular}
\end{table}

\begin{table}[!t]\small
	\centering 
	\caption{The convergence accuracy (\%) of models that are trained with different methods (FedDC and three baselines including FedAvg, Scaffold and FedDyn) on iid, non-iid and unbalanced data for full (100\%) client participating and part (15\%) participating. We also give the improvements on the accuracy of FedDC compared with FedAvg in the last column. 
	}
	\label{tab-best-accuracy-2}
	\begin{tabular}{|c|cccccc|}
		\hline
		\multicolumn{1}{|c|}{Data   distribution} &
		\multicolumn{1}{c|}{FedAvg} &
		\multicolumn{1}{c|}{FedProx} &
		\multicolumn{1}{c|}{Scaffold} &
		\multicolumn{1}{c|}{FedDyn} &
		\multicolumn{1}{c|}{FedDC} &
		Improvement \\ \hline\hline
		\multicolumn{7}{|c|}{100 clients 100\% participating}            \\ \hline
		MNIST-IID             & 98.12  & 98.12   & 98.32    & 98.51  & 98.45 & +0.33  \\ %\cline{1-1}
		MNIST-Dirichlet(0.3)   & 97.98  & 97.96   & 98.45    & 98.46  & 98.51 &  +0.53  \\ %\cline{1-1}
		MNIST-Dirichlet(0.6)   & 98.09  & 98.05   & 98.39    & 98.44  & 98.48 &  +0.39  \\
		MNIST-Unbalance    & 98.12  & 98.1    & 98.35    & 98.6   & 98.46 &  +0.34  \\ \cline{1-1}
		EMNIST-L-IID            & 94.82  & 94.66   & 95.64    & 95.3   & 95.55 &  +0.73 \\ %\cline{1-1}
		EMNIST-L-Dirichlet(0.3)  & 94.34  & 94.3    & 95.36    & 94.99  & 95.27 &  +0.93     \\ %\cline{1-1}
		EMNIST-L-Dirichlet(0.6) & 94.38  & 94.48   & 95.51    & 95.34  & 95.46 &  +1.08   \\ \hline\hline
		\multicolumn{7}{|c|}{100 clients 15\% participating}            \\ \hline
		MNIST-IID             & 98.15 & 98.11 & 98.45 & 98.38 & 98.47 &  +0.32  \\ 
		MNIST-Dirichlet(0.3)  & 98    & 98.04 & 98.37 & 98.3  & 98.4  &  +0.4   \\	%\cline{1-1}
		MNIST-Dirichlet(0.6)  & 98.13 & 98.12 & 98.49 & 98.3  & 98.49 &  +0.36  \\ 
		MNIST-Unbalance  	 & 98.15 & 98.13 & 98.5  & 98.34 & 98.5  &  +0.35  \\ \cline{1-1}
		EMNIST-L-IID            & 94.83 & 94.67 & 95.44 & 95.23 & 95.71 &  +0.88   \\ 
		EMNIST-L-Dirichlet(0.3) & 94.05 & 94.13 & 95.05 & 94.58 & 95    &  +0.95   \\ %\cline{1-1}
		EMNIST-L-Dirichlet(0.6) & 94.39 & 94.37 & 95.53 & 94.93 & 95.42 &  +1.03  \\ \hline\hline
		\multicolumn{7}{|c|}{100 clients 100\% participating}            \\ \hline
		Syn(0,0)              & 98.65 & 98.65 & 98.65 & 99.25 & 99.35 &  +0.7 \\ 
		Syn(1,0)             & 97.83 & 97.82 & 97.9  & 98.65 & 98.83 &  +1     \\ 
		Syn(0,1)             & 97.75 & 97.75 & 97.9  & 99.1  & 99.3  &  +1.55 \\ \hline
		\multicolumn{7}{|c|}{100 clients 15\% participating}            \\ \hline
		Syn(0,0)             & 98.75 & 98.7  & 98.65 & 99.32 & 99.57 &  +0.82\\ 
		Syn(1,0)            & 97.7  & 97.67 & 97.9  & 98.82 & 99.23 &  +1.53   \\ 
		Syn(0,1)             & 98.52 & 98.5  & 98.58 & 99.3  & 99.62 &  +1.1 \\ \hline
	\end{tabular}
\end{table}






\begin{figure}[!t]
	\centering 
	\subfigbottomskip=2pt
	\subfigcapskip=-5pt 
	\subfigure[]{
		\includegraphics[width=0.4\linewidth]{./nips-figs/F1.0/mnist_100_23_iid_alpha}}
	\subfigure[]{
		\includegraphics[width=0.4\linewidth]{./nips-figs/F0.15/cifar10_100_23_iid_alpha}}\\
	\subfigure[]{
		\includegraphics[width=0.4\linewidth]{./nips-figs/F1.0/mnist_100_23_iid_alpha_loss}}
	\subfigure[]{
		\includegraphics[width=0.4\linewidth]{./nips-figs/F0.15/cifar10_100_23_iid_alpha_loss}}
	\caption{Convergence plots of FedDC for different hyper-parameter-$\alpha$ settings with 100 clients adopting $100\%$ and $15\%$ client participating settings on iid MNIST and CIFAR10.}\label{figure_alpha}
\end{figure}


\begin{figure}[!t]
	\centering 
	\subfigbottomskip=2pt
	\subfigcapskip=-5pt 
	\subfigure[]{
		\includegraphics[width=0.4\linewidth]{./nips-figs/F0.15/ablation_iid}}
	\subfigure[]{
		\includegraphics[width=0.4\linewidth]{./nips-figs/F0.15/ablation_non_iid}}
	\caption{Ablation study for FedDC on CIFAR10. FedDC(le) adopts the proposed training process and uses the empirical loss as local objection function. FedDC(le+lp) adopts the proposed training process and uses the sum of the empirical loss and the parameter correction term as local objection function. FedDC(le+lg) adopts the proposed training process and uses the sum of the empirical loss and the gradient correction term as local objection function. FedDC(le+lg+lp) adopts the proposed training process and uses the sum of the empirical loss, the gradient correction term and the parameter correction term as local objection function.  }\label{figure_ablation}
\end{figure}

\begin{figure}[!t]
	\centering 
	\subfigbottomskip=2pt
	\subfigcapskip=-5pt 
	\subfigure[]{
		\includegraphics[width=0.4\linewidth]{./nips-figs/F0.15/syn_alpha-0_0_beta-0_0_theta_0_0_30_20_5_200_0_000000_0_000000_0_000000_True_True}}
	\subfigure[]{
		\includegraphics[width=0.4\linewidth]{./nips-figs/F1.0/syn_alpha-0_0_beta-0_0_theta_0_0_30_20_5_200_0_000000_0_000000_0_000000_True_True}}\\
	\subfigure[]{
		\includegraphics[width=0.4\linewidth]{./nips-figs/F0.15/syn_alpha-1_0_beta-0_0_theta_0_0_30_20_5_200_1_000000_0_000000_0_000000_True_True}}
	\subfigure[]{
		\includegraphics[width=0.4\linewidth]{./nips-figs/F1.0/syn_alpha-1_0_beta-0_0_theta_0_0_30_20_5_200_1_000000_0_000000_0_000000_True_True}}\\
	\subfigure[]{
		\includegraphics[width=0.4\linewidth]{./nips-figs/F0.15/syn_alpha-0_0_beta-1_0_theta_0_0_30_20_5_200_0_000000_1_000000_0_000000_True_True}}
	\subfigure[]{
		\includegraphics[width=0.4\linewidth]{./nips-figs/F1.0/syn_alpha-0_0_beta-1_0_theta_0_0_30_20_5_200_0_000000_1_000000_0_000000_True_True}}
	\caption{Convergence plots on Synthetic dataset. There are three types of settings, including the homogeneous setting where $(\gamma_1,\gamma_2)$ equal $(0,0)$, and two heterogeneous settings where $(\gamma_1,\gamma_2)$ equal $(1,0)$ and $(0,1)$, respectively.}\label{fig_syn}
\end{figure}

\begin{figure}[!t]
	\centering 
	\subfigbottomskip=2pt
	\subfigcapskip=-5pt 
	\subfigure[]{
		\includegraphics[width=0.4\linewidth]{./nips-figs/F0.15/mnist_100_23_iid__0_300000}}
	%\quad
	\subfigure[]{
		\includegraphics[width=0.4\linewidth]{./nips-figs/F1.0/mnist_100_23_iid__0_300000}}
	\subfigure[]{
		\includegraphics[width=0.4\linewidth]{./nips-figs/F0.15/CIFAR10_100_23_iid__0_300000}}
	\subfigure[]{
		\includegraphics[width=0.4\linewidth]{./nips-figs/F1.0/CIFAR10_100_23_iid__0_300000}}
	\\
	\subfigure[]{
		\includegraphics[width=0.4\linewidth]{./nips-figs/F0.15/CIFAR100_100_23_iid__0_300000}}
	%\quad
	\subfigure[]{
		\includegraphics[width=0.4\linewidth]{./nips-figs/F1.0/CIFAR100_100_23_iid__0_300000}}
	\caption{Convergence plots with 100 clients adopting $100\%$ and $15\%$ client participating settings on unbalanced data of MNIST, CIFAR10 and CIFAR100.}\label{figure_unbalance}
\end{figure}



\begin{figure}[!t]
	\centering 
	\subfigbottomskip=2pt
	\subfigcapskip=-5pt 
	\subfigure[]{
		\includegraphics[width=0.4\linewidth]{./nips-figs/F0.15/MNIST_100_23_iid_}}
	\subfigure[]{
		\includegraphics[width=0.4\linewidth]{./nips-figs/F1.0/MNIST_500_23_iid_}}
	\\
	\subfigure[]{
		\includegraphics[width=0.4\linewidth]{./nips-figs/F0.15/CIFAR10_100_23_iid_}}
	%\quad
	\subfigure[]{
		\includegraphics[width=0.4\linewidth]{./nips-figs/F1.0/CIFAR10_500_23_iid_}}
	\subfigure[]{
		\includegraphics[width=0.4\linewidth]{./nips-figs/F0.15/CIFAR100_100_23_iid_}}
	%\quad
	\subfigure[]{
		\includegraphics[width=0.4\linewidth]{./nips-figs/F1.0/CIFAR100_500_23_iid_}}
	\caption{Convergence plots for different number of clients adopting $100\%$ and $15\%$ client participating settings in the iid datasets of MNIST, CIFAR10 and CIFAR100.}\label{figure_client_number}
\end{figure}



\begin{figure}[!t]
	\centering 
	\subfigbottomskip=2pt
	\subfigcapskip=-5pt 
	\subfigure[]{
		\includegraphics[width=0.3\linewidth]{./nips-figs/F0.15/CIFAR10_100_23_iid_}}
	\subfigure[]{
		\includegraphics[width=0.3\linewidth]{./nips-figs/F0.15/CIFAR10_100_20_Drichlet_0_300.png}}
	\subfigure[]{
		\includegraphics[width=0.3\linewidth]{./nips-figs/F0.15/CIFAR10_100_20_Drichlet_0_600.png}}
	\\
	\subfigure[]{
		\includegraphics[width=0.3\linewidth]{./nips-figs/F1.0/CIFAR10_100_23_iid_}}
	%\quad
	\subfigure[]{
		\includegraphics[width=0.3\linewidth]{./nips-figs/F1.0/CIFAR10_100_20_Drichlet_0_300}}
	\subfigure[]{
		\includegraphics[width=0.3\linewidth]{./nips-figs/F1.0/CIFAR10_100_20_Drichlet_0_600}}
	\caption{Convergence plots for iid and non-iid data with 100 clients adopting $100\%$ and $15\%$ client participating settings on CIFAR10.}\label{figure_cifr10}
\end{figure}



\begin{figure}[!t]
	\centering 
	\subfigbottomskip=2pt
	\subfigcapskip=-5pt 
	\subfigure[]{
		\includegraphics[width=0.3\linewidth]{./nips-figs/F0.15/CIFAR100_100_23_iid_}}
	\subfigure[]{
		\includegraphics[width=0.3\linewidth]{./nips-figs/F0.15/CIFAR100_100_20_Drichlet_0_300.png}}
	\subfigure[]{
		\includegraphics[width=0.3\linewidth]{./nips-figs/F0.15/CIFAR100_100_20_Drichlet_0_600.png}}
	\\
	\subfigure[]{
		\includegraphics[width=0.3\linewidth]{./nips-figs/F1.0/CIFAR100_100_23_iid_}}
	%\quad
	\subfigure[]{
		\includegraphics[width=0.3\linewidth]{./nips-figs/F1.0/CIFAR100_100_20_Drichlet_0_300}}
	\subfigure[]{
		\includegraphics[width=0.3\linewidth]{./nips-figs/F1.0/CIFAR100_100_20_Drichlet_0_600}}
	\caption{Convergence plots for iid and non-iid data with 100 clients adopting $100\%$ and $15\%$ client participating settings on CIFAR100.}\label{figure_cifr100}
\end{figure}

\begin{figure}[!t]
	\centering 
	\subfigbottomskip=2pt
	\subfigcapskip=-5pt 
	\subfigure[]{
		\includegraphics[width=0.3\linewidth]{./nips-figs/F0.15/mnist_100_23_iid_}}
	\subfigure[]{
		\includegraphics[width=0.3\linewidth]{./nips-figs/F0.15/mnist_100_20_Drichlet_0_300.png}}
	\subfigure[]{
		\includegraphics[width=0.3\linewidth]{./nips-figs/F0.15/mnist_100_20_Drichlet_0_600.png}}
	\\
	\subfigure[]{
		\includegraphics[width=0.3\linewidth]{./nips-figs/F1.0/mnist_100_23_iid_}}
	%\quad
	\subfigure[]{
		\includegraphics[width=0.3\linewidth]{./nips-figs/F1.0/mnist_100_20_Drichlet_0_300}}
	\subfigure[]{
		\includegraphics[width=0.3\linewidth]{./nips-figs/F1.0/mnist_100_20_Drichlet_0_600}}
	\caption{Convergence plots for iid and non-iid data with 100 clients adopting $100\%$ and $15\%$ client participating settings on MNIST.}\label{figure_mnist}
\end{figure}


\begin{figure}[!t]
	\centering 
	\subfigbottomskip=2pt
	\subfigcapskip=-5pt 
	\subfigure[]{
		\includegraphics[width=0.3\linewidth]{./nips-figs/F0.15/emnist_100_23_iid_}}
	\subfigure[]{
		\includegraphics[width=0.3\linewidth]{./nips-figs/F0.15/emnist_100_20_Drichlet_0_300.png}}
	\subfigure[]{
		\includegraphics[width=0.3\linewidth]{./nips-figs/F0.15/emnist_100_20_Drichlet_0_600.png}}
	\\
	\subfigure[]{
		\includegraphics[width=0.3\linewidth]{./nips-figs/F1.0/emnist_100_23_iid_}}
	%\quad
	\subfigure[]{
		\includegraphics[width=0.3\linewidth]{./nips-figs/F1.0/emnist_100_20_Drichlet_0_300}}
	\subfigure[]{
		\includegraphics[width=0.3\linewidth]{./nips-figs/F1.0/emnist_100_20_Drichlet_0_600}}
	\caption{Convergence plots for iid and non-iid data with 100 clients adopting $100\%$ and $15\%$ client participating settings on EMNIST-L.}\label{figure_emnist}
\end{figure}





\begin{table}[!t]\small
	\centering
	\caption{The number of communication round in different methods to achieve a target accuracy while containing with $100$ clients which $100\%$ participating each round. The $SpeedUp$ factor is the number of communication round relative to FedAvg. }
	\label{tab_communication_saving}
	\begin{tabular}{|c|c|cccccc|}
		\hline
		\multirow{2}{*}{Method} &
		\multirow{2}{*}{Accuracy} &
		\multicolumn{2}{c|}{Non-iid (0.6-Dirichlet)} &
		\multicolumn{2}{c|}{Non-iid (0.3-Dirichlet)} &
		\multicolumn{2}{c|}{iid} \\ \cline{3-8} 
		&
		&
		\multicolumn{1}{c|}{Round} &
		\multicolumn{1}{c|}{SpeedUp} &
		\multicolumn{1}{c|}{Round} &
		\multicolumn{1}{c|}{SpeedUp} &
		\multicolumn{1}{c|}{Round} &
		SpeedUp \\ \hline
		\multicolumn{8}{|c|}{CIFAR10 $100$ clients $100\%$ participating} \\ \hline
		\multirow{1}{*}{FedAvg}  
		& 0.8  & \textgreater{}1000 & -        & \textgreater{}1000 & -    & 286 & -    \\ \hline
		\multirow{1}{*}{FedProx} 
		& 0.8  &  474   &  \textgreater{}2.11$\times$        & \textgreater{}1000    &      1$\times$ &  277   & 1.03$\times$     \\ \hline
		\multirow{1}{*}{Scaffold} 
		& 0.8  & 165 & >6.06$\times$ & 218 & >4.59$\times$  & 120 & 2.38$\times$   \\ \hline
		\multirow{1}{*}{FedDyn}  
		& 0.8  & 60  & >16.67$\times$    & 75  & >17.54$\times$ & 55  & 5.2$\times$    \\ \hline
		\multirow{1}{*}{FedDC}    
		& 0.8  & 53  & >18.86$\times$  & 70  & >14.28$\times$ & 43  & 6.65$\times$  \\ \hline\hline
		\multicolumn{8}{|c|}{CIFAR100 $100$ clients $100\%$ participating}               \\ \hline
		\multirow{1}{*}{FedAvg}  
		& 0.4  & 476 & -      & 847 & -    & \textgreater{}1000 & -    \\ \hline
		\multirow{1}{*}{FedProx} 
		&     0.4 & 502    &   0.95$\times$     &  507   &  1.67$\times$     &  273   & >3.66$\times$     \\ \hline
		\multirow{1}{*}{Scaffold} 
		& 0.4  & 91  & >5.23$\times$     & 94  & >9.01$\times$  & 84  & 11.9   \\ \hline
		\multirow{1}{*}{FedDyn}  
		& 0.4  & 51  & >9.33$\times$     & 53  & >15.98$\times$ & 56  & 17.85$\times$ \\ \hline
		\multirow{1}{*}{FedDC}    
		& 0.4  & 39  & >12.2$\times$     & 41  & >20.65$\times$ & 37  & 27.03$\times$ \\ \hline\hline
		\multicolumn{8}{|c|}{CIFAR10 $100$ clients $15\%$ participating} \\ \hline
		\multirow{1}{*}{FedAvg}  
		& 0.8  &616 & -        & \textgreater{}1000 & -     & \textgreater{}1000 & -       \\ \hline
		\multirow{1}{*}{FedProx} 
		& 0.8  &  459   & 1.34$\times$         &  \textgreater{}1000   &   1$\times$  &  307   &    \textgreater{}3.28   \\ \hline
		\multirow{1}{*}{Scaffold}
		& 0.8  & 200 & 3.08$\times$ & 263 & >3.80$\times$  & 126 & >7.93$\times$  \\ \hline
		\multirow{1}{*}{FedDyn}  
		& 0.8  & 193  & 3.19$\times$    & 195  & >5.12$\times$ & 145  & >6.9$\times$     \\ \hline
		\multirow{1}{*}{FedDC}   
		& 0.8  & 141  & 4.37$\times$  & 143  & >6.99$\times$ & 108  & >9.26$\times$  \\ \hline\hline
		\multicolumn{8}{|c|}{CIFAR100 $100$ clients $15\%$ participating}               \\ \hline
		\multirow{1}{*}{FedAvg}  
		& 0.4  & 615 & -        & 520 & -     & 724 & -     \\ \hline
		\multirow{1}{*}{FedProx} 
		&    0.4  &    980 &    0.63$\times$      &  503   &    1.03$\times$   & 650    &    >1.11$\times$    \\ \hline
		\multirow{1}{*}{Scaffold} 
		& 0.4  & 106  & 5.8$\times$     & 114  & 3.56$\times$  & 113  & 6.41$\times$  \\ \hline
		\multirow{1}{*}{FedDyn} 
		& 0.4  & 149  & 4.42$\times$     & 148  & 3.51$\times$ & 143  & 5.06$\times$   \\ \hline
		\multirow{1}{*}{FedDC}   
		& 0.4  & 102  & 6.03$\times$     & 103  & 5.05$\times$ & 100  & 7.04$\times$ \\ \hline\hline
		\multicolumn{8}{|c|}{MNIST $100$ clients $100\%$ participating} \\ \hline
		\multirow{1}{*}{FedAvg}  
		& 0.98  & 258               & -     & 492               &-          & 142               & -            \\ \hline
		\multirow{1}{*}{FedProx} 
		& 0.98  & 263               & 0.98$\times$  & 480               & 1.03$\times$        & 136               & 1.04$\times$ \\ \hline
		\multirow{1}{*}{Scaffold} 
		& 0.98  & 58                & 4.45$\times$ & 58                & 8.48$\times$  & 53                & 2.68$\times$\\ \hline
		\multirow{1}{*}{FedDyn} 
		& 0.98  & 46                & 5.61$\times$& 51                & 9.65$\times$  & 27                & 5.26$\times$\\ \hline
		\multirow{1}{*}{FedDC}     
		& 0.98   & 35                & 7.37$\times$& 37                & 13.3$\times$ & 26                & 5.46$\times$\\ \hline\hline
		\multicolumn{8}{|c|}{EMNIST-L $100$ clients $100\%$ participating}               \\ \hline
		\multirow{1}{*}{FedAvg}    & 0.94  & 142               &-  & 192               & -          & 107               & -           \\ \hline
		\multirow{1}{*}{FedProx}  & 0.94& 135               & 1.05$\times$  & 198               & 0.97$\times$    & 92                & 1.16$\times$   \\ \hline
		\multirow{1}{*}{Scaffold}  & 0.94 & 43                & 3.30$\times$& 52                & 3.69$\times$  & 30                & 3.57$\times$   \\ \hline
		\multirow{1}{*}{FedDyn}    & 0.94 & 30                & 4.73$\times$  & 52                & 3.69$\times$  & 27                & 3.96$\times$\\ \hline
		\multirow{1}{*}{FedDC}      & 0.94  & 43                & 3.3$\times$ & 60                & 3.2$\times$          & 21                & 5.1$\times$ \\ \hline\hline
		\multicolumn{8}{|c|}{MNIST $100$ clients $15\%$ participating} \\ \hline
		\multirow{1}{*}{FedAvg} 
		& 0.98     & 361               & -     & \textgreater{}600 & -         & 158               & -              \\ \hline
		\multirow{1}{*}{FedProx}  
		& 0.98 & 383               & 0.94$\times$ & 418               & \textgreater{}1.44$\times$  & 149               & 1.06$\times$\\ \hline
		\multirow{1}{*}{Scaffold} 
		& 0.98    & 62                & 5.82$\times$     & 72                &\textgreater{} 8.33$\times$  & 50                & 3.16$\times$  \\ \hline
		\multirow{1}{*}{FedDyn}  
		& 0.98  & 122               & 2.96$\times$ & 153               & \textgreater{}3.92$\times$ & 71                & 2.23$\times$ \\ \hline
		\multirow{1}{*}{FedDC}    
		& 0.98  & 60      & 6.02$\times$ & 62                &\textgreater{} 9.68$\times$           & 46                & 3.43$\times$ \\ \hline\hline
		\multicolumn{8}{|c|}{EMNIST-L $100$ clients $15\%$ participating}               \\ \hline
		\multirow{1}{*}{FedAvg}    & 0.94   & 153               & -       & 245               &-           & 108               & -         \\ \hline
		\multirow{1}{*}{FedProx}  & 0.94  & 145               & 1.06$\times$  & 240               & 1.02$\times$   & 105               & 1.03$\times$    \\ \hline
		\multirow{1}{*}{Scaffold} & 0.94   & 44                & 3.48$\times$ & 68                & 3.6$\times$& 42                & 2.57$\times$ \\ \hline
		\multirow{1}{*}{FedDyn}     & 0.94& 73                & 2.1$\times$  & 81                & 3.06$\times$        & 61                & 1.61$\times$ \\ \hline
		\multirow{1}{*}{FedDC}      & 0.94  & 48                & 3.19$\times$  & 74                & 3.31$\times$ & 47                & 2.3$\times$     \\ \hline
	\end{tabular}
\end{table}


